Exploiting Latent Attack Semantics for Intelligent Malware Detection

Behavioral malware detectors promise to expose previously unknown malware and are an important security primitive. However, even the best behavioral detectors suffer from high false positives and negatives. In this paper, we address the challenge of aggregating weak per-device behavioral detectors in noisy communities (i.e., ones that produce alerts at unpredictable rates) into an accurate and robust global anomaly detector (GD). Our system - Shape GD - combines two insights: Structural: actions such as visiting a website (waterhole attack) or membership in a shared email thread (phishing attack) by nodes correlate well with malware spread, and create dynamic neighborhoods of nodes that were exposed to the same attack vector; and Statistical: feature vectors corresponding to true and false positives of local detectors have markedly different conditional distributions. We use neighborhoods to amplify the transient low-dimensional structure that is latent in high-dimensional feature vectors - but neighborhoods vary unpredictably, and we use shape to extract robust neighborhood-level features that identify infected neighborhoods. Unlike prior works that aggregate local detectors' alert bitstreams or cluster the feature vectors, Shape GD analyzes the feature vectors that led to local alerts (alert-FVs) to separate true and false positives. Shape GD first filters these alert-FVs into neighborhoods and efficiently maps a neighborhood's alert-FVs' statistical shapes into a scalar score. Shape GD then acts as a neighborhood level anomaly detector - training on benign program traces to learn the ShapeScore of false positive neighborhoods, and classifying neighborhoods with anomalous ShapeScores as malicious. Shape GD detects malware early (~100 infected nodes in a ~100K node system for waterhole and ~10 of 1000 for phishing) and robustly (with ~100% global TP and ~1% global FP rates).

==> abstract.tex <==

WARNING!!!!

UNUSED.

ABSTRACT in paper.tex

% Anomaly-based intrusion detection systems promise to expose 
% previously unknown malware
% %i.e., new malware whose signatures are not yet present in malware databases,
% and thus form an important security primitive.
% %model benign applications' system calls and network traffic
% However, even the best anomaly detectors suffer from high false
% positives and are susceptible to mimicry attacks (where
% malware is deliberately crafted to look very similar to benign programs).

% In this paper, we address the challenge of composing noisy
% per-device local detectors into an accurate and robust global
% anomaly detector.  % Specifically, we propose to dynamically
% construct communities of local detectors and aggregate the local
% detector outputs in order to pin-point anomalous communities.
% Interestingly, since our global detector adapts to changes in
% underlying network to identify malware-infested neighborhoods
% dynamically, we do not have to place static observers on network
% nodes.  % We evaluate our technique on networks A, B, and C, where
% each node on the network is a mobile device running Android
% applications with real human user inputs, and find that our
% technique significantly improves the time to detection of new
% malware compared to a naive baseline. %by X\%
%
Behavioral malware detectors, by using statistical methods, promise to
expose previously unknown malware and thus form an important security
primitive. However, even the best detectors suffer from high false
positives and negatives.  In this paper, we address the challenge of
composing a community of weak per-device behavioral detectors (aka
local detectors) into an accurate and robust global anomaly detector.

Our system consists of feature-vector driven local detectors at
individual nodes; aggregating alerts (that flag the
possibility of malware being present) from this community of local
detectors enables global inference of malware.
%
% Specifically, we propose to dynamically construct communities of local
% detectors and aggregate the local detector outputs in order to
% pin-point anomalous communities.
%
%
Our system -- Shape GD -- combines two insights -- one structural and
the other statistical: {\em Structural:} actions such as visiting a
website (waterhole attack) or membership in a shared email thread
(phishing attack) by nodes
correlate well with malware spread
and creates a {\em neighbohood} of nodes; 
and {\em Statistical:} feature vectors corresponding
to true and false positives of local detectors have markedly different
conditional distributions (i.e. their histogram shapes differ).



% Crucially this
% property allows our global detector to be robust to noise in estimates
% of community size and data reporting behavior by individual users.


% \todo{We prototype our system on a community of Android devices.  Using 18
% different local detectors and 10 different malware tainted Android
% apps (AVG, Wikipedia, Yelp, etc.), we show, using a custom-built
% evaluation platform on which popular mobile applications are driven by
% real user inputs, that our global detector significantly improves
% malware detection probabilities in a variety of network settings.}

We evaluate Shape GD through emulation on a community of Windows
systems, where we collect data from a few thousand malware and benign
applications. We evaluate our system in the settings of a phishing
attack in a corporate setting, and a waterhole attack through a
popular website. In both these scenarios, we show that Shape GD
detects the presence of malware robustly, and at early stages of
infection.


% \item[3.] \textbf{Local/Global Detector Experiments:} We have
%   conducted experiments with 18 local detectors (random forest, SVM,
%   decision trees, ensemble methods, etc) and 10 Android apps
%   (Wikipedia, AVG, Walmart, Yelp, among others). First, we confirm the
%   premise that, on Android, a vast majority of local detectors' true
%   and false positive rates are about 80\%:15\% (see
%   Figure~\ref{fig:ROC}). Importantly, our key observation that the
%   conditional distributions differ at the global level, is borne out
%   by our experiments.  For 8 out of 10 apps, we observe a sharp
%   statistical separation between the scores resulting from the local
%   detector's TP and FP feature vectors. This manifests in the global
%   ROC curves: With 3000 samples fed to LDs and filtering by their
%   alerts, we can get a global TP:FP rates arbitrarily close to
%   100\%:0\% for 5 apps (AVG, Buzzfeed, All Recipes, Wikipedia, Zedge),
%   and about 95\%:5\% for two apps (see Figures~\ref{fig:GD_ROC} for
%   details of other apps). These can be further driven down
%   (theoretically, exponentially fast) by increasing the data set size.


% \item[4.] \textbf{Network Experiments:} We experiment with three
%   network topologies — grids, random graphs, and social network graphs
%   — and evaluate our global detector using standard generative models
%   for malware propagation on these graphs. The combination of shape
%   and censoring alerts enables malware to be detected when less than
%   10\% of the nodes are infected at false positive rate about 5\% (for
%   social network) and less than 1\% for the other networks with the
%   Wikipedia app (see Figure~\ref{fig:detect_vs_prctile}). Further, the number of
%   observations needed to detect at this level of reliability grows
%   only logarithmically with the network size (i.e., only a vanishingly
%   small fraction of the community need to report alerts, see
%   Figure~\ref{fig:wiki_vs_censoring_threshold}).


% Our global detector the presence of malware using (a) biased samples
% (self selection bias from local detectors) and the shape difference
% between the conditional distributions of FP feature vectors and TP
% feature vectors, and (b) alert censoring using thresholding based on
% graph-dependent alert densities. Crucially, this algorithm is robust
% to community size and data reporting dynamics, and the resulting
% variability in sample sizes.


% Interestingly, since our global detector adapts to changes in underlying
% network to identify malware-infested neighborhoods dynamically,  
% we do not have to place static observers on network nodes. 
% % 
% We evaluate our technique on networks A, B, and C, where each node on the
% network is a mobile device running Android applications with real human user
% inputs, and find that our technique significantly 
% improves the time to detection of new malware compared to a naive baseline. %by X\%




% \item[1.] \textbf{Algorithm:} We develop a novel global detector that
%   infers the presence of malware using (a) biased samples (self
%   selection bias from LDs) and the shape difference between the
%   conditional distributions of FP feature vectors and TP feature
%   vectors, and (b) alert censoring using thresholding based on
%   graph-dependent alert densities. Crucially, this algorithm is robust
%   to community size and data reporting dynamics, and the resulting
%   variability in sample sizes.

% \item[2.] \textbf{Platform:} We build a realistic evaluation platform
%   on which popular mobile applications are driven by real user inputs,
%   where we guarantee that a diverse set of malware payloads execute
%   correctly, and simulate a variety of network models for malware
%   propagation using a large network of emulators. \todo{number for
%     hours of sim and dataset}

% \item[3.] \textbf{Local/Global Detector Experiments:} We have
%   conducted experiments with 18 local detectors (random forest, SVM,
%   decision trees, ensemble methods, etc) and 10 Android apps
%   (Wikipedia, AVG, Walmart, Yelp, among others). First, we confirm the
%   premise that, on Android, a vast majority of local detectors' true
%   and false positive rates are about 80\%:15\% (see
%   Figure~\ref{fig:ROC}). Importantly, our key observation that the
%   conditional distributions differ at the global level, is borne out
%   by our experiments.  For 8 out of 10 apps, we observe a sharp
%   statistical separation between the scores resulting from the local
%   detector's TP and FP feature vectors. This manifests in the global
%   ROC curves: With 3000 samples fed to LDs and filtering by their
%   alerts, we can get a global TP:FP rates arbitrarily close to
%   100\%:0\% for 5 apps (AVG, Buzzfeed, All Recipes, Wikipedia, Zedge),
%   and about 95\%:5\% for two apps (see Figures~\ref{fig:GD_ROC} for
%   details of other apps). These can be further driven down
%   (theoretically, exponentially fast) by increasing the data set size.


% \item[4.] \textbf{Network Experiments:} We experiment with three
%   network topologies — grids, random graphs, and social network graphs
%   — and evaluate our global detector using standard generative models
%   for malware propagation on these graphs. The combination of shape
%   and censoring alerts enables malware to be detected when less than
%   10\% of the nodes are infected at false positive rate about 5\% (for
%   social network) and less than 1\% for the other networks with the
%   Wipikepdia app (see Figure~\ref{fig:detect_vs_prctile}). Further, the number of
%   observations needed to detect at this level of reliability grows
%   only logarithmically with the network size (i.e., only a vanishingly
%   small fraction of the community need to report alerts, see
%   Figure~\ref{fig:wiki_vs_censoring_threshold}).


==> accenture.tex <==
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/accenture/histogram/histogram.eps}\par
   \caption{Histogram of benign and malicious ShapeScores in an enterprise network: 
            The ShapeScore is computed
     from neighborhood sizes of 1,000 FVs (experiment repeated 100
     times to generate the histograms).  Though the histograms overlap,
     Shape-based GD can reliably flag some malicious neighborhoods.}
\label{fig:accenture-hist}
\end{figure}


We applied Shape GD to one month (February 2016) of security logs in a Fortune
500 enterprise. This dataset is extremely noisy and heterogeneous -- unlike our
homogeneous dataset in the paper which models deployments like {\tt osquery} in 
Facebook. In contrast, this dataset includes an average of 
almost 250 Million security-related log entries per day from almost 20 different local
detectors (Blue Coat, Symantec, McAfee, F5, Cisco, etc), generated from a system with over
150K devices (including personal computers, mobile devices, servers, firewalls,
routers, and other network elements), all recorded in a `market leading' SIEM
tool for global malware analysis. Devices come and go, log entries can be
delayed by up to two months, and logs with confirmed signature-based malware
infections are very rare (0.29\%). Hence, ground truth infection data is hard
to get. The goal here is to filter the 5.5 Billion log entries including 700,000
different server IPs in February 2016 to a few tens of incidents that can be manually
analyzed.



%We deployed Shape GD in a SIEM environment within Accenture company~\cite{accenture_company}
%and conducted preliminary experiments.
%Accenture's SIEM infrastructure stores logs collected across 100,000 devices over 
%a year long period; it contains 65 billions of log entries total.
%%Out of 200,000 reporting devices <?> are end hosts, the others are network
%%devices. 
%The data come from 18 different monitoring tools such
%ArcSight, Blue Coat, F5, Cisco and etc. Almost all end host devices 
%run antiviruses supplied by Symantec and Microsoft.
%
%For processing such enormous amount of data we choose Apache Spark~\cite{apache_spark},
%a large-scale data processing framework, which run
%in a cluster composed of 18 worker nodes equipped
%with 2.74 TB of RAM and 576 virtual cores.
%
%The way the data is organized imposes a set of new challenges that are
%orthogonal to the design of Shape GD, but affect its detection results.

First, the data is high-dimensional and sparse. Each log entry contains 468
categories filled out with mostly categorical values, and most rows have no
content or are filled out with uninformative default values. 
%The architects of Accenture's SIEM chose such a high-dimensional
%representation to unify logs reported by different tools that are not designed
%to work together.
Directly using one-hot encoding to represent categorical data produces a
330,000-dimensional vector, hence we use the top 20 security-critical
dimensions and encode data manually before applying one-hot encoding to yield
364 dimensional vectors. Determining unique identities for devices and
identifying usernames and domain-names associated with IP addresses in rows
takes several analysis passes over the sparse dataset.
%combination of manual encoding of data and ch whose dimensionality is a sum of
%the number of observed distinct values within each category. Obviously, such
%extreme dimensionality which is far beyond Spark's data processing
%capabilities. To address this challenge, we select only a subset of
%categories, perform manual feature encoding based on our expertise, and only
%after that we use one-hot encoding.  To speed up data processing, we have to
%stick to small number of categories (fewer than we would like to use), thus
%the resulting feature vectors have only 364 dimensions.
%
%The second challenge is matching log entries reported by different monitoring
%tools. Their logs may have inconsistent fields filled out, which prevents easy
%matching and requires to do multiple passes on the database to extract
%information. 
%
%
%: high-dimensional data, hard and expensive to correlate logs provided
%different tools, logs contain lots of missing or default values, and there is
%little documentation explaining what system events make all these monitoring
%tools generate log events. For example, one tool may report device's IP, while
%the other may fill it out with a loopback-address "127.0.0.1".  In this case,
%we have to extract user names associated with a specific set of IPs, and then
%query the database again to extract logs associated with those users.  The
%problem stems from the fact that the monitoring tools were not been designed
%or configured for large-scale data processing, instead, each of them reports
%its own data only.


%\textbf{Results}
%We obtained preliminary results by running Shape GD on one month of data --
%the data that was logged in Februrary 2016, the first month when the SIEM 
%became fully functional. This data subset includes 5.5 billion of log entries
%coming from 700,000 different IPs.% and 355,000 unique accounts.


We form neighborhoods based on the accessed domains, thus a neighborhood 
includes devices accessing different URLs hosted in the same domain. 
This yields 400,000 unique neighborhoods.
%Even such a coarse-grained neighborhood template leads to forming
%an enormous number of neighborhoods -- 400,000 unique neighborhoods.
%Such neighborhoods capture waterhole attacks and malware communication with
%its command and control servers.
We apply two heuristics to rank those neighborhoods in terms of their
maliciousness. First, we run SecureRank algorithm, 
which is an adaptation of PageRank algorithm for the problem
of ranking domains in terms of their potential maliciousness.
We initialize the SecureRank algorithm by labeling domains belonging to certain Blue Coat's
categories (e.g. Suspicious, Spam, Scam/Questionable/Illegal, etc) as malicious.
%The actual 'malicious' weight we assign depends on empirical observations that we 
%made when analyzing data.
SecureRank 
%converges fast to the final solution and 
outputs a sorted list of
domain names based on their malicious score.
%We manually checked some domains in the malicious part of the spectrum and
%discovered that 
%%they are not necessarily malicious, i.e. 
%SecureRank has high false positive rate.
%\mikhail{TODO: how much?}

%This is why we employ 
Our second heuristic is to query VirusTotal scanner to obtain
information about security incidents related to a particular domain.
VirusTotal's reports include the number of malicious URLs, the number of
malware samples communicating to a particular domain, the number of samples
embedding URL strings leading to the domain under investigation. If VirusTotal
does not have information about incidents related to a particular domain, then
we discard the domain from the list of suspicious domains (i.e., the candidates
for neighborhood formation process).
%We extracted end host alerts from the logs to validate the hypothesis whether
%those two heuristics are enough to conclude that a domain is compromised.  And
%it turns out that they have 
%Even filtering domains using VirusTotal yields an unacceptably high false
%positive rate.  \mikhail{TODO: How much?}

\noindent \textbf{Training Shape GD.} To build a reference histogram, we select the top
20 benign domains given by Secure Rank (and confirmed using VirusTotal),
aggregate all 31 Million log records related to communication with those
domains, and learn a reference vector-histogram.  The next step in the training
process is to determine threshold $\gamma$, which depends on the distribution
of benign neighborhood scores.  For this reason, we select the top 100 benign
domains from our domain list (not including the previously used 20 domains),
build neighborhoods for each domain, randomly select 1,000 records from each
neighborhood, and compute ShapeScore.  We select a thousand records because we
want our Shape GD to operate on domains that have more than a thousand records.
Thus, if during testing a domain's neighborhood yields less than a thousand
records, we have to discard it.  
%We experiment with three settings of the threshold $\gamma$ -- 97-th, 98-th, and 99-th percentiles.

{
\footnotesize
\begin{table}[htb]	
	\resizebox{\columnwidth}{!}{%
    \begin{tabular}{| l | l | l |}
    \hline
    $\gamma$, percentile & Flagged nbds & Prevented incidents \\ \hline
    97 & 25 & 15 \\
    98 & 15 & 11 \\
    99 & 5  & 7 \\  \hline
    \end{tabular}
    }
    \label{tbl:accenture_results}
   \caption{Shape GD prioritizing a total of 100 candidate neighborhoods and 30 confirmed exploits.}
%   	\caption{{\small \sf Running Shape GD on an enterprise's heterogeneous SIEM infrastructure. 
%      Shape GD takes as input the top 100 suspicious domains found using SecureRank and VirusTotal,
%      that generate a total to 30 alerts in the dataset. 
%   	We vary the threshold parameter $\gamma$ from 97th up to 99th percentile and observe that
%   	at 97 percentile, Shape GD flags only 25 neighborhoods/domains as malicious and yet pre-empt 15 of the 30
%      exploits.  
%      %and the number of 
%   	At 99 percentile, the prevented exploits drops from 15 to 7; however, the confidence that
%   	a flagged neighborhood is actually malicious increases.}}
\end{table}
}

\noindent \textbf{Testing Shape GD.} We select the top 100 {\em suspicious} domains
according to SecureRank followed by VirusTotal, form a neighborhood of end hosts using
each of these 100 domains,
select the first 1000 records in chronological order, 
%(we want to detect malware as soon as possible),
and run Shape GD. 
%Figure~\ref{fig:accenture-hist} shows the histogram of 
%ShapeScores generated by benign (blue bars) and malicious (red bars) neighborhoods.
%It is clear that malicious and benign neighborhoods' scores do not separate 
%as well as in our homogeneous system -- 
%the diversity of LDs and their feature vectors, and the sparsity
%of this dataset makes it an {\em extremely} challenging deployment point.
%In effect, the reduced detection rate implies that
%Yet, one can see that ShapeScore is discriminative enough to separate
%out a significant fraction of malicious neighborhoods. 


We experimented with three values of the threshold $\gamma$ -- 97th, 98th, 99th
percentiles (Table~\ref{tbl:accenture_results}). For each threshold we computed
the number of security incidents that could have been prevented during February
once Shape GD declares the domain (i.e.  its neighborhood) as infected.
%time period, this statistics is based on the number of end host alerts in our
%database.
These thresholds result in labeling 25, 15, and 5 domains/neighborhoods
(respectively) as infected, and yet pre-empt 15, 11, and 7 (respectively) of
the 30 exploits.  Increasing $\gamma$ from 97th percentile to 99th percentile
enables an analyst to trade off the number of domains that need to be
manually analyzed with the number of exploits that were pre-empted.

%but increases Shape GD's discriminative ability
%from 3$\times$ up to 7$\times$ (the ratio of the fraction of domains that an
%analyst needs to check to the fraction of exploits that she will prevent).


%We analyzed the end hosts that access those hosts in February and counted the number
%of alerts that the end host protection system raised when an end host accessed one
%of those domains. Such an estimate is very conservative in the sense that the end host 
%protection system might have raised an alert or blocked a sample when malware
%was performing local actions without trying to access the Internet.

%In the far right column -- ShapeScore -- we can easily spot an outlier domain
%{\tt j.maxmind.com}.  Its ShapeScore is 2--3 times higher than the threshold.
%On querying VirusTotal, we found out that this domain has hosted 57 malicious
%URLs, 100 malware samples have communicated with this domain and 100 samples
%embed this domain in their strings.  

%Based on the data in the SIEM data base,
%seven users had malware communicating to this host in February alone {\em
%after} Shape GD had raised an alert. 

%Shape GD could have reliably spotted this domain
%name and if the incident response team had processed the results fast enough, at least
%seven infections could have been prevented.

%For each value of $\gamma$ threshold we compute the number of incidents that could 
%have been prevented, the same parameter per each flagged neighborhood and for each 
%unflagged neighborhood (the last two lines in the table). And we see 

%We are still working on increasing of Shape GD's accuracy when applying it to the
%existing SIEM infrastructures, and also we are working on co-design of
%SIEM infrastructures and Shape GD to achieve the best possible detection rate.


%\begin{table}[htb]	
%	\resizebox{\columnwidth}{!}{%
%    \begin{tabular}{| l | l | l | l |}
%    \hline
%    Parameter & $\gamma$ = 97th prctile & $\gamma$ = 98th prctile &
%				$\gamma$ = 99th prctile \\ \hline
%	Flagged neighborhoods & 25 & 15 & 5 \\
%	Prevented incidents & 15 & 11 & 7 \\
% 	Shape GD's discriminative ability & 3x & 3.3x & 5.8x \\ \hline
%    \end{tabular}
%    }
%    \label{tbl:accenture_results}
%   	\caption{Running Shape GD in Accenture's SIEM infrastructure. 
%   	For each neighborhood, we show results for three values of the threshold
%   	$\gamma$ -- 97th, 98th, and 99th percentiles. The values in the corresponding
%   	column shows the number of infected user accounts whose infections could be 
%   	prevented if had Shape GD been deployed in the beginning of 2016.}
%\end{table}

%\begin{table}[htb]	
%	\resizebox{\columnwidth}{!}{%
%    \begin{tabular}{| l | l | l | l | l |}
%    \hline
%    Domain name & $\gamma$ = 97th & $\gamma$ = 98th &
%				$\gamma$ = 99th  & ShapeScore \\ \hline
%    j.maxmind.com & 7 & 7 & 7 & 67.74\\ 
%	grarhibck.com & 0 & 0 & 0 & 42.06\\ 
%	mashable.com & 0 & 0 & 0 & 36.42\\ 
%	delivery.adforgecdn.com & 0 & 0 & 0 & 29.50\\ 
%	beacon.securestudies.com & 0 & 0 & 0 & 28.81\\ 
%	tools.dvdvideosoft.com & 0 & 0 &  & 27.84\\ 
%	videolan.org & 0 & 0 &  & 26.91\\ 
%	euwfb.adsrvr.org & 1 & 1 &  & 26.25\\ 
%	t12.baidu.com & 1 & 1 &  & 25.98\\ 
%	creative.ad120m.com & 0 & 0 &  & 25.83\\ 
%	serve.popads.net & 1 & 1 &  & 25.48\\ 
%	yui.yahooapis.com & 0 & 0 &  & 25.44\\ 
%	sovrn-merge.openx.net & 0 & 0 &  & 25.30\\ 
%	cm.pos.baidu.com & 1 & 1 &  & 25.24\\ 
%	eclick.baidu.com & 0 & 0 &  & 25.09\\ 
%	bkrtx.com & 0 &  &  & 24.13\\ 
%	c.fqtag.com & 0 &  &  & 24.12\\ 
%	groupon.com & 0 &  &  & 24.03\\ 
%	xp.apple.com & 1 &  &  & 23.85\\ 
%	platform.stumbleupon.com & 0 &  &  & 23.71\\ 
%	cpro.baidu.com & 1 &  &  & 23.43\\ 
%	oz.cnzz.com & 0 &  &  & 23.19\\ 
%	go.oclasrv.com & 1 &  &  & 22.71\\ 
%	arcadeparlor.com & 0 &  &  & 22.70\\ 
%	letterboxd.com & 1 &  &  & 22.58\\ \hline \hline
%	Prevented incidents & 15 & 11 & 7 & \\ \hline
% 	Prevented incidents per nbd & 0.60 & 0.73 & 1.40 &  \\ \hline 
% 	Incidents per missed nbd & 0.20 & 0.22 & 0.24 &  \\ \hline 
%    \end{tabular}
%    }
%    \label{tbl:accenture_results}
%   	\caption{Running Shape GD in Accenture's SIEM infrastructure. 
%   	For each neighborhood, we show results for three values of the threshold
%   	$\gamma$ -- 97th, 98th, and 99th percentiles. The values in the corresponding
%   	column shows the number of infected user accounts whose infections could be 
%   	prevented if had Shape GD been deployed in the beginning of 2016.}
%\end{table}


==> discussion_main_text.tex <==
\noindent \textbf{Global FPs vs LD FPs.} As remarked in the Introduction, an FP
of 1\% at the global level means that we will see one alert every 100 - 300
hours (for the phishing scenario) and 100 seconds (for waterhole scenario 
the neighborhood time window slides by 1 second). This reduces work to 
be performed by the deeper, second-level analysis considerably.

Specifically, LDs operating at 6\% false positive rate generate 23.5M -- 70M
FPs within 100--300 hours time interval in a network of 1086 nodes (phishing)
and 300K alerts within every 100 sec interval where neighborhoods include
$\sim$50K nodes on average (waterhole). Shape GD filters these alerts.  When
using 1--3 hours (phishing) and 6 sec (waterhole) time-based neighborhood
filtering, Shape GD will report to a system running a deeper analysis
approximately 234.5K -- 703.7K FPs raised by LDs (phishing) and approximately
1.4K FPs (waterhole).  Adding structural filtering brings these numbers down to
21.6K -- 64.8K FPs (phishing) and 360 FPs (waterhole).

Compared to a neighborhood of LDs, Shape GD thus reduces  the number of FPs
reported to deeper analyses by $\sim$100$\times$ and $\sim$200$\times$ when
employing time-based filtering only (for phishing and waterhole scenarios
respectively), while structural filtering reduces alert-FVs for deeper analysis
to $\sim$1000$\times$ and $\sim$830$\times$.
%by $\sim10\times$ and $\sim4\times$ correspondingly Shape GD reports 
%Note that the waterhole scenario gains less from structural filtering than
%phishing because structural filtering leads to an increase in neighborhood time
%window (in waterhole scenario) from 6 second up to 25 second, adding many more
%benign FVs per neighborhood.  
In both scenarios, analysts can choose to reduce
number of alert-FVs to be analyzed by sliding neighborhood windows by a larger
interval; however, this will increase the time to detect malware infection.

% \noindent \textbf{Templates for unknown attacks.}  \mikhail{We make an
%   assumption that for each known network-level attack it is possible
%   to define a neighborhood formation template based on the semantics
%   of an
%   attack.%, i.e. the rules to aggregate nodes into a neighborhood.
%   Since the number of network-level attacks (e.g. waterhole, phishing
%   and etc) is reasonable, then development of an individual template
%   for each attack is a feasible process that is performed only once.
%   Once a new attack is detected, a corresponding template needs to be
%   developed, however, new attack types do not emerge frequently.  }

% \noindent \textbf{What if FPs and TPs are indistinguishable?}
% \mikhail{
% One may challenge the main assumption about distinguishability of FP and TP distributions, 
% which forms the basis for Shape GD.
% They can be indistinguishable only if LDs are perfect, i.e. they extract all useful 
% information from the data. However, machine learning algorithms often involve solving NP-hard 
% problems, and to accomplish this they fall back on using various heuristics. 
% Therefore, it is very unlikely for practical machine learning algorithms to retrieve all the 
% information from the underlying data. As a consequence, their FPs and TPs bear information 
% allowing Shape GD to separate them.
% }

==> experimental-setup/appStatsTableProcessed.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{p{1.3cm} p{1.5cm} c c c c c c c c c c}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{File Ops} & \multicolumn{2}{c}{Network Ops} & \multicolumn{2}{c}{Process Ctrl} & \multicolumn{2}{c}{System Wide} &\multicolumn{2}{c}{Misc} \\
App & Config & $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$\\\hline
Allrecipes&Benign&8.08e+02&3.78e+02&1.97e+00&1.56e+02&0.00e+00&1.77e+03&3.53e+02&1.06e+01&2.05e+02&0.00e+00\\
Allrecipes&File stealer&3.12e+03&2.12e+00&7.76e+02&2.37e+02&1.97e+02&6.26e+03&5.17e+00&1.63e+03&4.93e+02&5.81e+02\\
Allrecipes&Contacts stealer&3.29e+03&2.47e+00&8.67e+02&2.69e+02&2.31e+02&6.39e+03&5.74e+00&1.81e+03&5.40e+02&6.89e+02\\
Allrecipes&SMS stealer&3.12e+03&2.14e+00&7.49e+02&2.29e+02&2.05e+02&6.76e+03&5.24e+00&1.54e+03&4.69e+02&6.34e+02\\
Allrecipes&Other stealer&3.34e+03&2.40e+00&8.97e+02&2.73e+02&2.49e+02&6.30e+03&5.40e+00&1.76e+03&5.19e+02&7.79e+02\\
Allrecipes&Click fraud&3.32e+03&2.30e+00&8.21e+02&2.52e+02&2.19e+02&6.30e+03&5.29e+00&1.62e+03&4.78e+02&6.62e+02\\
Allrecipes&GET flood&3.13e+03&2.26e+00&7.85e+02&2.44e+02&1.91e+02&6.14e+03&5.41e+00&1.47e+03&4.73e+02&5.35e+02\\
Allrecipes&SHA1- cracker&3.08e+03&2.29e+00&8.27e+02&2.48e+02&2.20e+02&6.31e+03&5.43e+00&1.74e+03&5.00e+02&6.88e+02\\ 
\hline
AVG&Benign&3.39e+02&1.71e+01&5.10e+00&1.72e+02&1.31e-02&7.51e+02&5.57e+01&4.31e+01&1.49e+02&1.84e-01\\
AVG&File stealer&2.79e+03&2.93e+01&1.40e+03&3.91e+02&3.18e+02&3.99e+03&2.01e+01&1.20e+03&4.18e+02&1.04e+03\\
AVG&Contacts stealer&3.01e+03&2.91e+01&1.25e+03&3.99e+02&3.24e+02&4.22e+03&1.96e+01&1.37e+03&4.52e+02&1.01e+03\\
AVG&SMS stealer&3.03e+03&2.88e+01&1.30e+03&3.96e+02&3.68e+02&3.95e+03&1.96e+01&1.20e+03&4.10e+02&1.26e+03\\
AVG&Other stealer&2.68e+03&2.76e+01&1.62e+03&3.89e+02&3.58e+02&4.76e+03&2.03e+01&1.53e+03&6.02e+02&1.16e+03\\
AVG&Click fraud&3.13e+03&2.95e+01&1.07e+03&4.06e+02&2.78e+02&4.03e+03&2.17e+01&1.16e+03&4.52e+02&9.58e+02\\
AVG&GET flood&3.26e+03&3.04e+01&1.03e+03&4.01e+02&3.14e+02&3.82e+03&1.95e+01&9.16e+02&3.69e+02&1.04e+03\\
AVG&SHA1- cracker&2.80e+03&2.79e+01&1.49e+03&4.03e+02&3.28e+02&3.89e+03&1.87e+01&1.34e+03&3.95e+02&1.12e+03\\
\hline
The Bible&Benign&2.22e+02&1.51e+01&1.92e+00&2.12e+02&1.98e-04&1.88e+02&1.43e+01&5.21e+00&1.31e+02&2.67e-02\\
The Bible&File stealer&1.08e+03&4.00e+01&1.02e+03&3.11e+02&2.62e+02&9.19e+02&2.37e+01&6.87e+02&2.55e+02&4.63e+02\\
The Bible&Contacts stealer&1.26e+03&4.21e+01&8.84e+02&3.13e+02&2.49e+02&9.59e+02&5.90e+01&7.25e+02&2.46e+02&3.86e+02\\
The Bible&SMS stealer&1.27e+03&4.18e+01&8.71e+02&3.09e+02&2.45e+02&1.12e+03&2.91e+01&7.54e+02&3.03e+02&4.50e+02\\
The Bible&Other stealer&1.08e+03&3.95e+01&1.14e+03&3.20e+02&2.77e+02&1.16e+03&2.75e+01&7.78e+02&3.13e+02&4.74e+02\\
The Bible&Click fraud&1.45e+03&4.27e+01&7.41e+02&3.23e+02&2.52e+02&1.07e+03&3.15e+01&7.40e+02&2.92e+02&4.84e+02\\
The Bible&GET flood&1.38e+03&4.20e+01&7.38e+02&3.11e+02&2.27e+02&8.12e+02&2.07e+01&6.32e+02&1.89e+02&4.27e+02\\
The Bible&SHA1- cracker&1.16e+03&4.06e+01&9.77e+02&3.09e+02&2.50e+02&9.44e+02&5.51e+01&7.09e+02&2.43e+02&4.27e+02\\
\hline
Buzzfeed&Benign&5.04e+02&3.52e+01&4.93e+00&3.00e+02&0.00e+00&4.71e+02&3.71e+01&8.19e+00&5.91e+02&0.00e+00\\
Buzzfeed&File stealer&3.92e+03&2.58e+01&1.26e+03&3.49e+02&2.06e+02&4.39e+03&1.52e+01&1.31e+03&2.53e+02&3.96e+02\\
Buzzfeed&Contacts stealer&3.83e+03&2.38e+01&1.48e+03&3.84e+02&2.65e+02&4.29e+03&1.45e+01&1.34e+03&2.99e+02&4.62e+02\\
Buzzfeed&SMS stealer&3.65e+03&2.41e+01&1.64e+03&3.51e+02&2.95e+02&4.23e+03&1.45e+01&1.56e+03&2.85e+02&6.88e+02\\
Buzzfeed&Other stealer&3.16e+03&2.26e+01&2.03e+03&3.21e+02&4.33e+02&3.60e+03&1.37e+01&1.74e+03&2.11e+02&1.01e+03\\
Buzzfeed&Click fraud&3.62e+03&1.95e+01&1.73e+03&4.24e+02&3.17e+02&4.33e+03&1.31e+01&1.32e+03&3.44e+02&5.02e+02\\
Buzzfeed&GET flood&4.31e+03&2.43e+01&1.24e+03&3.70e+02&1.77e+02&4.75e+03&1.45e+01&1.17e+03&3.10e+02&3.58e+02\\
Buzzfeed&SHA1- cracker&3.56e+03&2.22e+01&1.64e+03&3.57e+02&2.12e+02&4.04e+03&1.36e+01&1.42e+03&2.89e+02&3.51e+02\\
\hline
eBay&Benign&7.12e+01&1.00e+01&1.93e+00&1.54e+02&0.00e+00&6.73e+01&1.11e+01&7.55e+00&1.12e+02&0.00e+00\\
eBay&File stealer&1.77e+03&5.36e+01&9.12e+02&6.97e+02&1.85e+02&1.35e+03&3.27e+01&7.89e+02&4.83e+02&1.61e+02\\
eBay&Contacts stealer&1.75e+03&5.15e+01&9.67e+02&6.76e+02&1.85e+02&1.31e+03&2.96e+01&8.27e+02&4.30e+02&1.69e+02\\
eBay&SMS stealer&1.86e+03&5.12e+01&9.29e+02&6.70e+02&1.76e+02&1.56e+03&3.56e+01&8.96e+02&5.20e+02&1.89e+02\\
eBay&Other stealer&1.71e+03&5.24e+01&9.88e+02&6.84e+02&1.84e+02&1.46e+03&3.28e+01&8.96e+02&4.96e+02&1.60e+02\\
eBay&Click fraud&1.78e+03&5.16e+01&9.16e+02&6.83e+02&1.81e+02&1.23e+03&2.99e+01&8.03e+02&4.40e+02&1.78e+02\\
eBay&GET flood&1.74e+03&5.26e+01&9.78e+02&7.02e+02&1.99e+02&1.44e+03&3.36e+01&9.18e+02&5.26e+02&2.29e+02\\
eBay&SHA1- cracker&1.84e+03&5.31e+01&9.41e+02&6.92e+02&1.88e+02&1.44e+03&3.08e+01&8.53e+02&4.57e+02&2.22e+02\\
\hline
Html5 Ref.&Benign&5.19e+01&7.87e+00&3.30e+00&1.25e+02&1.94e-02&6.77e+01&1.05e+01&3.18e+01&2.04e+02&1.90e-01\\
Html5 Ref.&File stealer&1.06e+03&2.00e+00&6.53e+02&9.64e+01&1.01e+02&2.07e+03&6.81e+00&1.03e+03&3.46e+02&2.18e+02\\
Html5 Ref.&Contacts stealer&7.32e+02&1.85e+00&4.44e+02&5.81e+01&1.01e+02&1.06e+03&6.39e+00&6.57e+02&1.59e+02&1.97e+02\\
Html5 Ref.&SMS stealer&7.63e+02&2.08e+00&4.67e+02&6.53e+01&1.14e+02&1.04e+03&6.63e+00&5.70e+02&1.70e+02&2.28e+02\\
Html5 Ref.&Other stealer&7.95e+02&2.22e+00&4.64e+02&6.21e+01&1.14e+02&1.08e+03&6.81e+00&5.27e+02&1.65e+02&2.11e+02\\
Html5 Ref.&Click fraud&7.44e+02&1.69e+00&4.54e+02&6.56e+01&1.04e+02&1.07e+03&6.05e+00&5.47e+02&1.66e+02&2.10e+02\\
Html5 Ref.&GET flood&6.18e+02&1.32e+00&4.25e+02&6.70e+01&9.64e+01&9.15e+02&5.32e+00&5.88e+02&1.61e+02&1.93e+02\\
Html5 Ref.&SHA1- cracker&7.64e+02&1.71e+00&4.52e+02&6.10e+01&1.01e+02&1.10e+03&6.10e+00&5.73e+02&1.66e+02&2.05e+02\\
\hline
\end{tabular}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{p{1.3cm} p{1.5cm} c c c c c c c c c c}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{File Ops} & \multicolumn{2}{c}{Network Ops} & \multicolumn{2}{c}{Process Ctrl} & \multicolumn{2}{c}{System Wide} &\multicolumn{2}{c}{Misc} \\
App & Config & $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$\\\hline
Walmart&Benign&1.34e+02&9.97e+00&1.56e+00&1.21e+02&0.00e+00&1.34e+02&1.31e+01&6.50e+00&1.01e+02&0.00e+00\\
Walmart&File stealer&1.94e+03&3.14e+01&1.31e+03&2.97e+02&3.09e+02&1.41e+03&2.26e+01&1.14e+03&1.86e+02&5.83e+02\\
Walmart&Contacts stealer&1.95e+03&3.15e+01&1.26e+03&3.00e+02&3.06e+02&1.40e+03&2.29e+01&1.09e+03&2.28e+02&4.79e+02\\
Walmart&SMS stealer&2.19e+03&3.23e+01&1.11e+03&3.01e+02&2.72e+02&1.42e+03&2.24e+01&1.10e+03&1.81e+02&4.48e+02\\
Walmart&Other stealer&1.86e+03&3.14e+01&1.49e+03&2.96e+02&3.36e+02&1.58e+03&2.39e+01&1.11e+03&2.18e+02&5.96e+02\\
Walmart&Click fraud&2.23e+03&3.33e+01&1.09e+03&3.11e+02&2.96e+02&1.48e+03&2.34e+01&1.10e+03&2.15e+02&4.88e+02\\
Walmart&GET flood&1.96e+03&3.08e+01&1.24e+03&2.94e+02&3.04e+02&1.58e+03&2.20e+01&1.08e+03&1.91e+02&5.25e+02\\
Walmart&SHA1- cracker&2.07e+03&3.18e+01&1.19e+03&2.96e+02&2.87e+02&1.43e+03&2.37e+01&1.22e+03&1.90e+02&4.54e+02\\
\hline
Wikipedia&Benign&5.97e+01&4.30e+00&1.27e+00&5.23e+01&1.73e-04&1.81e+02&1.25e+01&1.10e+01&1.49e+02&1.56e-02\\
Wikipedia&File stealer&1.16e+02&4.66e-02&1.15e+02&9.86e+00&7.49e+01&1.38e+02&7.63e-01&1.20e+02&2.35e+01&1.09e+02\\
Wikipedia&Contacts stealer&1.16e+02&3.83e-02&1.15e+02&9.57e+00&7.54e+01&1.35e+02&6.71e-01&1.17e+02&2.25e+01&1.12e+02\\
Wikipedia&SMS stealer&1.15e+02&4.62e-02&1.15e+02&9.39e+00&7.66e+01&1.34e+02&7.50e-01&1.23e+02&1.96e+01&1.22e+02\\
Wikipedia&Other stealer&1.15e+02&3.84e-02&1.14e+02&9.36e+00&7.47e+01&1.33e+02&6.69e-01&1.20e+02&1.77e+01&1.06e+02\\
Wikipedia&Click fraud&1.18e+02&4.35e-02&1.17e+02&9.66e+00&7.57e+01&1.46e+02&7.16e-01&1.21e+02&2.19e+01&1.10e+02\\
Wikipedia&GET flood&1.18e+02&4.14e-02&1.16e+02&1.01e+01&7.65e+01&1.41e+02&6.57e-01&1.19e+02&2.43e+01&1.21e+02\\
Wikipedia&SHA1- cracker&1.15e+02&4.82e-02&1.15e+02&9.57e+00&7.48e+01&1.35e+02&7.44e-01&1.19e+02&2.21e+01&1.12e+02\\
\hline
Yelp&Benign&1.43e+02&3.17e+01&5.95e+00&1.56e+02&9.35e-04&1.50e+02&3.89e+01&4.04e+01&1.48e+02&5.36e-02\\
Yelp&File stealer&3.54e+02&1.63e+00&2.55e+02&9.10e+01&1.78e+02&9.30e+02&2.09e+01&7.25e+02&2.62e+02&4.08e+02\\
Yelp&Contacts stealer&1.76e+02&7.23e-01&1.28e+02&4.58e+01&9.76e+01&7.15e+02&4.19e+00&4.91e+02&1.77e+02&2.94e+02\\
Yelp&SMS stealer&1.87e+02&7.70e-01&1.34e+02&4.73e+01&1.01e+02&6.81e+02&4.18e+00&4.74e+02&1.64e+02&2.99e+02\\
Yelp&Other stealer&1.66e+02&6.90e-01&1.29e+02&4.69e+01&1.02e+02&5.02e+02&3.92e+00&4.81e+02&1.62e+02&2.99e+02\\
Yelp&Click fraud&1.87e+02&7.82e-01&1.38e+02&4.82e+01&1.01e+02&8.92e+02&4.39e+00&5.05e+02&1.84e+02&2.96e+02\\
Yelp&GET flood&1.91e+02&7.57e-01&1.37e+02&4.84e+01&1.06e+02&6.71e+02&4.27e+00&4.66e+02&1.69e+02&3.19e+02\\
Yelp&SHA1- cracker&1.70e+02&6.91e-01&1.27e+02&4.37e+01&9.41e+01&6.82e+02&3.90e+00&4.84e+02&1.64e+02&2.88e+02\\
\hline
Zedge&Benign&9.33e+01&3.40e+00&1.97e+00&1.50e+02&7.41e-05&8.92e+01&6.59e+00&9.67e+00&1.15e+02&8.61e-03\\
Zedge&File stealer&1.48e+03&4.73e+01&1.10e+03&2.97e+02&2.20e+02&1.96e+03&2.59e+01&7.06e+02&2.61e+02&3.26e+02\\
Zedge&Contacts stealer&1.65e+03&4.58e+01&9.78e+02&3.09e+02&2.54e+02&2.00e+03&2.30e+01&7.77e+02&2.40e+02&4.60e+02\\
Zedge&SMS stealer&1.64e+03&4.61e+01&9.43e+02&2.93e+02&2.13e+02&1.89e+03&2.32e+01&7.18e+02&2.06e+02&3.52e+02\\
Zedge&Other stealer&1.39e+03&4.50e+01&1.27e+03&2.90e+02&2.47e+02&2.28e+03&2.39e+01&9.45e+02&2.61e+02&4.21e+02\\
Zedge&Click fraud&1.97e+03&4.61e+01&7.84e+02&3.16e+02&2.05e+02&2.20e+03&3.01e+01&8.27e+02&3.05e+02&3.81e+02\\
Zedge&GET flood&1.88e+03&4.66e+01&7.94e+02&3.00e+02&1.94e+02&2.19e+03&2.78e+01&7.11e+02&2.70e+02&3.14e+02\\
Zedge&SHA1- cracker&1.53e+03&4.55e+01&1.10e+03&3.04e+02&2.20e+02&1.85e+03&2.20e+01&7.62e+02&2.19e+02&3.48e+02\\
\hline
\end{tabular}
\end{table*}


==> experimental-setup/malware-propogation-model.tex <==
The malware propogation model follows an exponential distrub ...

This is similar to some tuberculosis infection models \sanjay{PLEASE CITE}

==> experimental-setup/small-stats-table.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{p{1.3cm} p{1.7cm} c c c c c c c c c c}
\multicolumn{2}{c}{} & \multicolumn{2}{c}{File Ops} & \multicolumn{2}{c}{Network Ops} & \multicolumn{2}{c}{Process Ctrl} & \multicolumn{2}{c}{System Wide} &\multicolumn{2}{c}{Misc} \\
App & Config & $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$& $\mu$ & $\sigma$\\\hline
Wikipedia&Benign&59.71&4.30&1.27&52.27&0.00&181.11&12.49&10.96&148.95&0.02\\
Wikipedia&Info Stealers&115.88&0.04&115.10&9.61&75.48&135.56&0.73&120.09&21.74&113.02\\
Wikipedia&Click fraud&118.18&0.04&116.65&9.66&75.66&145.88&0.72&120.79&21.91&109.86\\
Wikipedia&GET flood&117.90&0.04&116.38&10.08&76.51&140.62&0.66&119.14&24.29&121.10\\
Wikipedia&SHA1 cracker&115.47&0.05&115.00&9.57&74.81&135.24&0.74&118.96&22.11&111.52\\
\hline
Yelp&Benign&142.71&31.71&5.95&156.44&0.00&150.31&38.91&40.37&148.35&0.05\\
Yelp&Info Stealers&246.35&1.08&178.53&63.70&129.87&787.28&13.37&590.97&210.95&345.86\\
Yelp&Click fraud&186.80&0.78&137.90&48.21&100.56&891.92&4.39&504.53&183.96&296.34\\
Yelp&GET flood&190.54&0.76&136.63&48.37&105.58&671.18&4.27&465.84&168.69&319.15\\
Yelp&SHA1 cracker&169.80&0.69&126.89&43.68&94.08&681.62&3.90&484.41&163.90&288.38\\
\hline \\
\end{tabular}
\caption{Mean, $\mu$, and standard deviation, $\sigma$, of system call intensities per second per logical group of system calls.}
\end{table*}


==> experimental-setup/synthetic-malware-gen.tex <==
% Synthetic Malware Generation 
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/tables/synthetic_malware.pdf}\par
\caption{\textit{(Synthetic malware payloads used in our experiments: 4 info stealers, 2 networked nodes, and 1 compute node. The settings represent a small fraction, but computationally diverse, set of malware behaviors.}}
\label{fig:synthetic-malware}
\end{figure}
%After many unsuccessful attempts to run real malware in our experimental setup, we reimplemented malicious functionality in the form of synthetic malware and use it throughout the paper. Carefully crafted synthetic malware benchmark is designed to closely resemble real-world malware and to provide precise control over its parameters. Also, synthetic malware includes a futuristic feature not seen in the wild -- it can lower its intensity to remain unnoticed by local detectors.

%After in-depth analysis of hundreds of mobile malware samples in the wild, we
%have come up with a new methodology that is a few steps ahead of the current
%approach to evaluation of malware detectors -- this is the most crucial
%component of our experimental setup.

We evaluate our GD algorithms not against off-the-shelf malware
whose ,
but also against advanced malware that tries to escape detection by
diversifying its payloads' executions. We describe the scope of malware behaviors
and our process to construct a state-of-the-art malware sample that is
guaranteed to execute correctly.

%hiding behind the variations of benign executions.
%Instead of testing the \sysname against old malware, we have developed a
%We begin with an off-the-shelf malware sample -- Geinimi.a
%benchmark that extends existing malicious behaviors by including the new ones
%-- not seen in the wild -- in order to be more powerful in breaking the
%detection schema.

\noindent {\bf Limitations of off-the-shelf malware.} Most malware samples
available
online~\cite{dissect_malware_2012,contagiodump,malware.lu,virusshare.com} do
not execute correctly. This is because malware often require older, vulnerable
versions of Android OS; they are designed to run only in a specific
geographical location; they include anti-emulation
defenses~\cite{anti_emulation_android_vidas}; they passively wait for commands
from command and control (C\&C) servers that are temporarily or permanently
down; or are programmed to react to specific user actions.  Another challenge
of using off-the-shelf malware is that
%understand malicious behavior that stands behind 
malware code-names assigned by anti-virus (AV) companies -- like
\textit{CruseWin} and \textit{AngryBirds-LeNa.C} -- do not inform an analyst
what payload the malware actually executes. 

Hence we evaluate our detector against malware that we have reverse-engineered
and ensured to work correctly (on both the device and C\&C server sides); whose
payloads we understand in behavioral terms (such as stealing files or
Contacts); and whose payloads we actively diversify to stress our detector.

%Moreover, sticking to a handful of malware samples that are able to
%run in a lab environment is likely to introduce bias into the experimental
%results because such malware samples usually do not exhibit complex behavioral
%patterns due to being trivially simple.
%\mohit{rephrase, please}
%After in-depth analysis of hundreds of mobile malware samples in the wild, we have come up with a new methodology that is a few steps ahead of the current approach to evaluation of malware detectors -- this is the most crucial component of our experimental setup.
%
%We have performed rigorous evaluation of our system not only against existing malicious behaviors, but also against advanced malware trying to escape from the local detectors by hiding behind the variations of benign executions.  Instead of testing the \sysname against old malware, we have developed a benchmark that extends existing malicious behaviors by including the new ones -- not seen in the wild -- in order to be more powerful in breaking the detection schema.
%
%\noindent {\bf Off-the-shelf malware.}
%Plenty of malware samples available online~\cite{dissect_malware_2012,contagiodump,malware.lu,virusshare.com} do not execute 'properly'. Malware may require older, vulnerable versions of Android OS, run only in a specific geographical location, include anti-emulation defenses~\cite{anti_emulation_android_vidas}, passively wait for commands from command and control (C\&C) servers that are temporarily or permanently have been brought down, react to specific user actions. Moreover, sticking to a handful of malware samples that are able to run in a lab environment is likely to introduce bias into the experimental results because such malware samples usually do not exhibit complex behavioral patterns due to being trivially simple.

%The main issue with malware samples available online~\cite{dissect_malware_2012,contagiodump,malware.lu,virusshare.com} is that they often do not execute 'properly'. Malware may require older, vulnerable versions of Android OS, run only in a specific geographical location, include anti-emulation defenses~\cite{anti_emulation_android_vidas}, passively wait for commands from command and control (C\&C) servers that are temporarily or permanently have been brought down, react to specific user actions. Moreover, sticking to a handful of malware samples that are able to run in a lab environment is likely to skew the resulting data set because such malware samples usually do not perform complex actions, thus we would not be able to observe complex malicious behaviors.

Another challenge coming from the blind use of off-the-shelf malware is to understand malicious behavior that stands behind obfuscated malware names assigned by an anti-virus (AV) company. For example, malware names like \textit{CruseWin} and \textit{AngryBirds-LeNa.C} do not inform an analyst what an expected malicious behavior is. 
%they should expect from those samples. 
Finally, inconsistency between naming conventions used by different AV companies aggravates the problem.

\noindent {\bf Malware design pattern.}
When designing synthetic malware, we have applied client-server paradigm that is common across all real-world malware samples. Malware running on a device performs malicious actions in response to the commands that it receives from its C\&C server and communicates back to the server to confirm successful completion. Synthetic malware allows numerous network-related parameters to be fine-tuned: frequency of communication with C\&C, network bandwidth, the size of data packets sent by client side, interpacket delays between them, device-level intensity of malicious actions.

The client-side code is organized using delegation software design pattern together with Android message passing interface. When a client receives a notification from C\&C in the form of an xml file, it parses server's request, configures itself and launches one or more Android services responsible for carrying out a malicious task. Depending on C\&C's request, malware may run those services sequentially or concurrently. Some services act as an intermediate dispatcher -- they perform initialization and then spawn parallel threads to conduct actual malicious activity asynchronously. For example, the service performing click fraud activity creates a thread pool and supplies a list of URL links to the workers in the pool that they must access.

It is worth noting that most Android apps (both benign and malicious) are obfuscated using standard Android tool -- Proguard~\cite{proguard}. It renames classes, fields, and methods with obscure names. We have applied Progaurd to the synthetic malware as well.

\noindent {\bf Variety of malicious behaviors.}
As a starting point for modeling diversity of malicious behaviors, we have analyzed 229 malware samples in 126 families, which cover prevailing mobile malware over last three years, that we have downloaded from the public repositories~\cite{contagiodump,malware.lu,virusshare.com}. We have identified common malicious behaviors and trends and reimplemented them closely following design of a reverse-engineered Geinimi sample~\cite{geinimi}.

%\noindent {\bf Malware design pattern.}
%When designing our synthetic malware, we have applied client-server paradigm that is common across all real-world malware samples. Malware running on a device performs malicious actions in response to the commands that it receives from its C\&C server and communicates back to the server to confirm successful completion. Synthetic malware allows numerous network-related parameters to be fine-tuned: frequency of communication with C\&C, network bandwidth, the size of data packets sent by client side, interpacket delays between them, device-level intensity of malicious actions.
%
%The client-side code is organized using delegation software design pattern together with Android message passing interface. When a client receives a notification from C\&C in the form of an xml file, it parses server's request, configures itself and launches one or more Android services responsible for carrying out a malicious task. Depending on C\&C's request, malware may run those services sequentially or concurrently. Some services act as an intermediate dispatcher -- they perform initialization and then spawn parallel threads to conduct actual malicious activity asynchronously. For example, the service performing click fraud activity creates a thread pool and supplies a list of URL links to the workers in the pool that they must access.
%\input{experimental-setup/malware-table}%

At a high level, client-side malicious code can perform several independent tasks that fall into one of the three behavioral categories that we have found when analyzing real malware samples: information stealers, networked nodes, and compute nodes. C\&C server may instruct client-side code to execute any combination of these basic tasks. Their implementation is described later in this section.

\noindent {\bf Information stealers.}
Malware stealing personal information usually focuses on accessing the following data: contacts for spamming purposes, text messages for breaking two-factor authentication (e.g. bank trojans), location and files on device for spying on users, phone IDs for legitimizing stolen devices. Our synthetic malware can easily model all these behaviors.

Contact stealing service is mainly governed by two parameters: the number of contacts being exfiltrated and delay between sending queries to the contact provider. 

As for SMS stealing behavior, real malware samples come in two flavors: batch and intelligent stealers (e.g. bank trojans). The former transmit all the text messages to their C\&C server, while the latter register an Android listener to intercept incoming SMS messages and scan them for the presence of authentication codes, alternatively they can perform intelligent text search within the database of already received messages and upload to the C\&C server only interesting ones.

As mentioned earlier, for spying purposes malware frequently accesses location information and steal files from a device, mostly photos. Following Android programming model, synthetic malware can obtain location by registering an Android listener that receives location updates or directly from Android middleware. In the latter case, OS returns a previously cached location that may have been determined using cellular network (approximate mode) or GPS (precise mode) if it is available on a device.

Our malware supports all basic file operations: it can send directory content, upload a particular file or several files to the C\&C server or store a file received from a server on a device. The latter functionality is widely used by malware developers to install new (likely malicious) apps.

The last type of malware steals device IDs such as IMEI and IMSI codes, OS info available via the static class android.os.Build and other miscellaneous device specific data such as browsing history and bookmarks, description of installed apps, call logs. Generally this information -- especially IMEI and IMSI -- can be used for impersonating purposes, in particular, to legitimize stolen devices before selling them on a black market, or for targeted advertising.

Our implementation of these functional blocks allows to specify the following parameters: amount of data being read (e.g. 1 or 10 contacts/SMSs/files), intensity of data accessing operations (e.g. read a file by 1K chunks), delay between successive reading operations (e.g. sleep for 100 ms between retrieving subsequent contacts/SMSs).

\noindent {\bf Networked nodes.}
The other behavioral malware category -- networked nodes -- includes mobile malware that exploits phone's network resources. It is getting more and more widespread as network bandwidth keeps rising up. Malware developers are lured by frequently changing device's IP and the ease of distributing malicious activity across many network nodes (devices) that are unlikely to be blacklisted. 

We have identified two types of an abuse of phone's network capabilities: click fraud and DDoS attacks~\cite{malware_blackhat_15, prolexic_q4_2013, android_ddos_2012}. Click fraud is one of the most popular ways of generating revenue out of having access to compromised hosts. Malicious service receives a list of URLs from a C\&C, periodically fetches webpages specified in the URL list and traverses their DOM structure. To speed up the process, our malware may launch several parallel threads.

The other type -- DDoS attacks from compromised mobile devices -- are getting more popular. Vast majority of DDoS attacks abuse HTTP protocol (e.g. 80\% according to \cite{ddos_threat_spectrum_2012}). Our malware is able to mount two attacks: GET flood and SlowLoris~\cite{slowloris_ddos}. GET flood comprises a series of GET requests sent by compromised network nodes. As opposed to GET flood, SlowLoris attack is far less computationally expensive because it tries to exhaust server pool of available connections by opening numerous connections and sending data very slowly to keep connections alive over a long time period. In our experiments, synthetic malware establishes 500 connections. If some connections fail, they are automatically reopened to keep the total number of active connections constant.

\noindent {\bf Compute nodes.}
The last category of malicious behaviors includes computationally intensive malware. Unlike the previous two, it may or may not leave distinguishable fingerprint at system call interface. A typical example of such malware is a bitcoin miner \cite{mobile-bitcoin-miner}. We approximate this category by the code cracking SHA1 passwords.

\noindent {\bf Realistic user data.}
In addition to careful modeling of malicious behaviors, we have invested a lot of efforts into populating our emulators with synthetic data that is statistically close to the real user data. For these purposes, we have followed the guidelines from the following empirical study~\cite{morpheus-hasp}. Without user data even a perfectly working malware may not perform anything malicious if, for example, it is designed to steal  data (e.g. photos, contacts, text messages and etc).

\noindent {\bf Repackaging Android apps.}
We have embedded synthetic malware into benign underlying apps using the same methods as malware developers: disassembled an apk using \textit{apktool}, copied malicious code into the apk, modified \textit{Manifest.xml} to extend the list of required permissions and to statically register malicious components. Finally, we have reassembled the decompiled app with \textit{apktool} and signed with \textit{jarsigner}.

\noindent {\bf Check for correctness.}
One of the key design decisions that we have made is to augment malware with capability to  notify data collection system when certain events happen (e.g. C\&C request has been successfully parsed, malware starts/finishes execution). This is very important because android emulators often crash, thus we can identify and rerun failed experiments. We also use malware start and stop time stamps to start and stop collecting malicious feature vectors.  We also make sure that the notification mechanism does not pollute the collected data.

\mikhail{we need a table with malware parameters + one paragraph to describe them}





==> intro/behavioral-analysis.tex <==
% Behavioral Analysis
\subsection{Behavioral Analysis}

\comment{

* Crowdroid Anomaly Detector
* Andromaly Anomaly Detector
* pBMDS: Anomaly Detector
* Behavioral Detection of Malware on Mobile Handsets: Anomaly Detector
* SmartSiren: Anomaly Detector: CIDS: network based
* Monitoring Smartphones for Anomaly Detection: Symbian: Features sent to remote server: Features == amount of free RAM, user inactivity, number of running processes, CPU utilization, SMS sent count

* A Layered Architecture for Detecting Malicious Behaviors: Behavioral Signature mining
* Synthesizing Near-Optimal Malware Specifications from Suspicious Behaviors: Behavioral Signature Mining
* Automated Classification and Analysis of Internet Malware: Behavioral Signature Mining

Anomaly Detection
Power based

In \cite{Schmidt2008}, Schmidt et al proposed an anomaly detection system based on Symbian. Due to mobile phone requirements, the authors sent the feature vectors to a remote server for processing. The features included amount of free RAM, a user inactive boolean, the number of running processes, the current CPU utilization, and the number of sent SMS messages.  

% Early Work
In \cite{Jacoby2004} authors monitored instantaneous current of a battery


Anomalous behavior detection systems attempt to statistically distinguish malicious activity from \emph{normal} benign execution. Once trained, behavioral classification engines determine whether a given feature vector is benign or suspicious, and emits a label accordingly. This implies that the feature set captures some abstract notion of program execution. For example, a commonly chosen, and relatively low level, feature is the system call trace\todo{DO THE LIST CITATIONS HERE}. System calls are provided by the OS and enable general programs to request OS services (open/close files, process management, etc.). For instance, Crowdroid, an early Android CIDS, treated system calls as a bag of words where each feature vector is simply a system call histogram per appli.   

Dynamic behavioral analysis techniques monitor program execution... 

Signals
System Calls + w params / API Calls \cite{Wagner:2002:MAH:586110.586145,Christodorescu:2008:MSM:1342211.1342215,kruegel2007,Fredrikson2010,Canali2012,Burguera2011,Kolbitsch:2009:EEM:1855768.1855790,Xie2010, rieck2008} 
Network Info \cite{Cheng2007,Roesch1999,staniford-chen1996,porras1997}
Battery/CPU\cite{Schmidt2008}/MEM\cite{Schmidt2008}/etc \cite{Buennemeyer2008,Jacoby2004,Kim2008}
Power\cite{clark2013}

Features:
N-Grams \cite{Gu2008,Canali2012}
Tuple \cite{Shabtai2012,Canali2012}
Bag \cite{Burguera2011,Canali2012, rieck2008}
Graph (Probably Dependency Graph or Approx) \cite{Christodorescu:2008:MSM:1342211.1342215,Kolbitsch:2009:EEM:1855768.1855790,Lippmann2008,Xie2010,kruegel2007}

Algorithms:
Histogram Comparison: \cite{Shabtai2012}
Classification (SVM, Clustering, etc) 
- kMeans: \cite{Burguera2011,Shabtai2012}
- kNN: \cite{Demme2013}
- ANN: \cite{Demme2013}
- SVM: \cite{rieck2008}
- Logistic Regression \cite{Shabtai2012}
- Decision Trees + Bayesian Networks \cite{Shabtai2012,Demme2013} 
HMMs \cite{Xie2010}
Graph Comparison \cite{Lippmann2008,kruegel2007}
Results

\begin{itemize}
% Classification (SVM, Clustering, etc) 
\item kMeans: \cite{Burguera2011,Shabtai2012}
\item kNN: \cite{Demme2013}
\item ANN: \cite{Demme2013}
\item SVM: \cite{rieck2008}
\item Logistic Regression \cite{Shabtai2012}
\item Decision Trees + Bayesian Networks \cite{Shabtai2012,Demme2013} 
\end{itemize}
}


Behavioral analysis refers to statistical methods that monitor signals from
program execution, extract features and build models from these signals, and
then use these models to classify processes as malicious.  Importantly, as we
discuss in this section, all known behavioral detectors have a high false
positive and negative rate (especially when zero-day and mimicry
attacks are factored in). 

%such as system calls, network traffic, instruction-level
%behavior etc, 

% System calls and parameters have been studied extensively
%Signals for behavioral analysis include
System-calls and middleware API calls have been studied extensively 
as a signal 
%are very commonly used signals 
for behavioral detectors~\cite{Wagner2002,Christodorescu:2008:MSM:1342211.1342215,kruegel2007,Fredrikson2010,Canali2012,Burguera2011,Kolbitsch:2009:EEM:1855768.1855790,Xie2010,
rieck2008,bose2008,Mutz2006,Forrest1996,Hofmeyr1998,Warrender1999,Somayaji2000}.
%Specifically for Android, Crowdroid\cite{Burguera2011} 
%uses system call traces sourced from
%several devices as the sole signal in its anomaly detection.  
Network intrusion 
detection systems like Snort, Bro~\cite{paxson1999}
HIDE~\cite{zhang2001}, EMERALD~\cite{porras1997}, BotSniffer~\cite{Gu2008}, and 
NetBiotic \cite{vlachos2004} analyze network traffic to detect known malicious
or anomalous behaviors.
More recently, behavioral detectors use signals such as power
consumption\cite{clark2013,Buennemeyer2008,Kim2008}, CPU
utilization\cite{Schmidt2008}, memory footprint\cite{Schmidt2008}, and hardware
performance counters\cite{Demme2013,Tang2014}. Specifically on 
Android, Andromaly\cite{Shabtai2012}
uses power consumption and CPU utilization, in addition to syscalls,
network flow, and control flow, as signals that are
tracked at runtime.


%Features go Here Rather than just saying whats popular, lets talk about how
%these features are useful in the statistical model building process Up the
%citation count
Detectors then extract {\em features} from these raw signals.  For example, an
n-gram is a contiguous sequence of n items that 
%is useful for their simplicity and their ability to 
captures total order relations~\cite{Gu2008,Canali2012}, n-tuples are ordered
events that do not require contiguity, and bags are simply histograms.
%Note, the dimensionality of the feature space is directly proportional to the
%value of n, however this comes at the expense of increased complexity and
%memory requirements. Dimensionality these features to compress the feature
%space into a smaller form that remains representative.  N-tuples are a strict
%relational ordering of n-grams, without requiring contiguity. n-tuples are
%useful in non-trivial combinations of
These can be combined to create bags of tuples, tuples of bags, and tuples of
n-grams~\cite{Shabtai2012,Canali2012,Forrest1996,Hofmeyr1998,Warrender1999}
often using principal component analysis to reduce dimensions.
%Bags are simply an unordered count of their contents. For example, bags may
%contain n-grams, tuples, or simply the original signal. Bags are useful
%because they describe the data in terms of its frequency
%distribution~\cite{Canali2012}. %Notable examples To reduce dimensions,
%analysts uses techniques such as include~\cite{Burguera2011,Canali2012,
%rieck2008,Warrender1999}. Rieck et al.~\cite{rieck2008} proposed a framework
%for automatically classifying malware samples into groups with similar
%behaviors.  
Further, system calls with their arguments form a dependency graph structure 
%spatio-temporal relations among features.  As~\cite{Canali2012} pointed out,
%complex combinations of N-grams, Tuples, and Bags can approximate these
%graphs. However, there are algorithms from graph
that can be compared to sub-graphs that represent malicious
behaviors~\cite{Christodorescu:2008:MSM:1342211.1342215,Kolbitsch:2009:EEM:1855768.1855790,Lippmann2008,Xie2010,kruegel2007}.
%theory that are useful for comparing graphs and subgraphs



% Anomaly start by listing overlapping methods Talk about hardware performance
% counters in the signals section
%Anomaly detection research use many different algorithms to extract alerts
%from
Finally, detectors train models to classify executions into malware/benignware
using supervised (signature-based) or unsupervised (anomaly-based) learning.
These models range from distance metrics~\cite{Forrest1996, Hofmeyr1998}, histogram
comparison~\cite{Kind2009}, hidden markov
models(HMM)~\cite{Xie2010,Warrender1999}, and neural networks (artificial neural
networks, fuzzy neural networks, etc. )~\cite{Demme2013,Wei2014}, to 
more common classifiers such as
%classification 
kNN\cite{Demme2013}, one-class SVMs~\cite{Tang2014},
decision trees\cite{Demme2013}, and ensembles thereof. 
%Andromaly evaluates histogram comparison, k-Means, logistic regression,
%decision trees, and baysian networks algorithms for its anomaly detection. 
\ignore{
pBMDS\cite{Xie2010} use HMMs to correlate
%probabilistic approach to anomaly detection by 
user inputs with system calls, whereas Xu et al.~\cite{Xu2004} apply sequence
alignment techniques to known and unknown malicious binaries to detect
polymorphic strains.
}

%Results
%Mobile platforms face resource limitations not evident in their PC
%counterparts. Although smartphones have become more powerful in recent years,
%minimizing analysis and detection overheads is still a top priority. Host-based

Such machine learning models, however, result in high false positives and
negatives.  
Anomaly detectors can be circumvented by mimicry attacks where
malware mimics system-calls of benign applications~\cite{Wagner2002} or
hides within the diversity of benign network traffic\cite{Sommer2010}.
Sommer et al.~\cite{Sommer2010} additionally highlights 
several problems that can arise due
to overfitting a model to a non-representative training set, suggesting signature-based
detectors as the primary choice for real deployments. Unfortunately, 
signature-based detectors cannot detect new (zero-day) attacks.
%show how mimicry attacks can circumvent system-call based detectors.
%Similarly, 
Specific to Android, both system
calls~\cite{Burguera2011} and hardware-counter based
detectors~\cite{Demme2013} 
%results for hardware performance counters to detect
yield $\sim$20\% false positives and $\sim$80\% true positives.

Our work {\em assumes} that each individual {\em local detector} (LD) is weak
and presents (a) a new property -- the different shapes of true- and
false-positive feature vectors -- and (b) a new censorship algorithm to
concentrate the weak signal in LDs' outputs.

%Our work can use any of the above detectors as {\em local detectors} (LDs)
%and 

%demonstrate that network traffic models are not robust to benign variations --
%leading to high false positives and `real' deployments working only with
%signature based detectors. 

%Intrusion detection systems such as Andromaly have managed to keep processing
%overheads at around 10\% with reasonable detection rates; Best case detection
%rates for Andromaly changed per experiment with TP/FP rates ranging from
%99.9\%/0.00\% to 85.3\%/16.2\%. Note, however, the Andromaly experiments use a
%few simple custom-written Android malware since no known Android malware
%existed. Alternatively, systems like Crowdroid choose to extract system call
%features locally, which is a lightweight task, and perform analysis in the
%cloud. The server computes a bag of system calls per execution trace and
%distinguishes malicious activity from benign activity using 2 cluster k-Means.
%The authors evaluate Crowdroid with a combination of 3 in-house apps and real
%malware samples; namely the Steamy Window app with PJApps Malware and Monkey
%Jump 2 with HongTouTou Malware. Given 60 execution traces per app, 50 benign
%and 10 malicious, the Crowdroid engine achieved 100\% TP and 0\% FP rates for
%all apps except Monkey Jump 2 which achieved 85\% detection with 3 false
%positives. The contrast between PJApps and HongTouTou detection rates is a
%byproduct of their intended malicious activities. PJApps launches a background
%application with many functions whereas HongTouTou just browses web pages and
%leaks phone information to a remote entity. In a sense, HongTouTou is stealthy
%compared to PJApps strains.        
        


%Discussion
%Talk about intended activity of malware and how this relates to intelligent malware. Talk about how sufficient data is needed to prevent overfitting in data mining pipeline.



==> intro/cids.tex <==
\subsection{Collaborative Intrusion Detection Systems (CIDS)}
\label{sec:cids}

% Can You infect me now?
% Malware Propagation in Large Scale Networks
% Smartphone Malware and Its Propagation Models: A Survey
% Modeling Malware Propagation in Smartphone Social Networks
% Why mobile-to-mobile Malware wont cause a storm
% BIG: Modeling and Restraining Mobile Virus Propagation


%Intrusion detection systems (IDS) monitor local or network operations for
%suspicious activities. 
Collaborative intrusion detection systems (CIDS) provide an architecture where
LDs' alerts are aggregated by a {\em global detector} (GD).
%correlate information across many per-device local detectors of these
%intrusion \emph{monitors}, improving the detection of intelligent local
%attacks. In particular, local detectors emit a stream of alerts and network
%overlays allow the system to determine neighborhoods.  The global detector
%takes the local detector streams and the neighborhoods from the network
%overlays and correlates the local detectors' alerts, considering only a
%neighborhood at a time.  Local Detector
GDs can use either signature-based\cite{kannadiga2005, snapp1991, cuppens2002,
yegneswaran2004, ramachandran2004, duma2006},
anomaly-based\cite{zhang2001,staniford-chen1996,vlachos2004}, or a combination
of the two~\cite{porras1997,krugel2001,paxson1999} to generate global alerts.
%Signature-based detectors are similar to malware detectors in that ther are
%unable to address unknown attacks. Anomaly detectors, however, are able to
%handle unknown attacks but usually suffer from a high false positive rate.
%Simple local detectors such as those in DIDS\cite{snapp1991} and
%DIDMA\cite{kannadiga2005} throw labeled flags for all suspicious activity
%(e.g. failed login attempts, modification of system files, telnet usage,
%rlogin usage, etc.). On the other hand, systems like HIDE\cite{zhang2001} emit
%statistical alerts in the form of random variables.
Additionally, the CIDS architecture can be centralized~\cite{porras1997},
hierarchical~\cite{zhang2001}, or distributed (using a peer-to-peer overlay
network)~\cite{yegneswaran2004,ramachandran2004,vlachos2004,duma2006,ZhouCV2005}.

%% Network Overlays
%\ignore{
%CIDSs use network overlays to determine inclusion or non-inclusion of specific
%nodes in the correlation analysis. Therefore, the networks are defined
%\emph{virtually} as a set of nodes logically connected via edges, for example a
%virtual graph may be constructed from the edges of a social network of friends
%and an email contact graph.
%}
%
%\ignore{
%The HIDE\cite{zhang2001} system assigns static network overlays
%hierarchically based on network locality. Global detectors in HIDE monitor machines on
%their local area network for suspicious activity and generate statistical
%reports based on their findings. These summaries are forwarded to, and aggregated
%at a global detector in the next level of the hierarchy. Note that this global
%detector is also monitoring its \emph{local} network for suspicious activity.
%
%Distributed CIDSs, which have neither a central processing component nor a strict
%hierarchical ordering, use network overlays to locate a neighborhood of nearby
%peers for alert correlation.
% Oftentimes, this mapping takes form as P2P
%networks~\cite{yegneswaran2004,ramachandran2004,vlachos2004,duma2006}.
%INDRA\cite{Janakiraman2003} uses a distributed hash table for organizing their
%global detectors in its P2P network overlays. In the LarSID
%system\cite{ZhouCV2005}, nodes \emph{subscribe} to network overlays, where they
%\emph{publish} suspicious findings. Therefore, all nodes serve as both local and
%global detectors.
%}


%Global detectors act as \emph{correlation engines} for a neighborhood of local
%detectors. One common paradigm for global detectors 

In all cases, existing GDs use some variant of count-based algorithms to
aggregate LDs' alerts \cite{Dash2006,Seurat2004}: once the number of alerts
exceeds a threshold within a space-time window, the GD raises an intrusion
alert. In HIDE~\cite{zhang2001}, 
%uses a multi-tiered system where 
the global detector at each hierarchical-tier is a neural network trained on
network traffic information.  Worminator\cite{Locasto2005} additionally uses
bloom filters to compact LDs' outputs and schedules LDs to form groups in order
to spread alert information quickly through a distributed system.  
All count based algorithms are fragile when the noise is high (in the early 
stages of an infection) and when the network size is uncertain.
%Our GD uses shape information and dynamically censors the output
In contrast, our shape and censoring based GD is robust against 
such uncertainty.

%We focus on early stage detection of zero-day infections and on
%aggregating alerts in 
%a network where the membership information is unreliable. 

Note that distributed CIDSs are vulnerable to probe-response attacks, where the
attacker probes the network to find the location and defensive capabilities of
an LD~\cite{Shmatikov2007,Bethencourt2005,Shinoda2005}. These attacks are orthogonal to our
setting since we do not have fixed LDs (i.e. all nodes act as LDs). 
 
%and generate global
%a network scheduling approach, implemented as
%a bloom filter, 
%to ensure that neighboring nodes with access to complementary
%pieces of information can communicate at approximately the same time.  
%This
%allows the system to determine if a local alert is simply noise or part of a
%distributed alert.


==> intro/global-d.tex <==
\subsection{Global Detectors}

\noindent \textbf{Count:} {\em Count} refers to the simple yet natural
idea that the number of alerts when there truly is a new malware in
the community differs from the baseline number of alerts. As our
results show, count provides statistical separation, but {\em only
  once the malware spread becomes large enough}; in the early stages,
the number of true alerts is drowned in the (comparatively) vast
number of false positive alerts. Thus, for early stage detection, we
seek something more powerful than count alone.

% For example, if the false positive rate is
% $0.3,$ and the true positive rate is $0.7,$

% To illustrate these, consider for concreteness, a
% community of 1000 nodes connected according to a typical social graph
% \cite{}. Assume that the local detectors at the individual nodes have
% false positive (misclassifies benign as malware) and false negative
% (misclassifies malware as benign) rates of $0.3.$

% \noindent \textbf{Count:} Count simply means that that number of
% alerts when there truly a malware in the community differs from the
% baseline count. Indeed, in our example, due to false positives, even
% when thereis no malware in the network, we expect $300 \pm 43$ (for
% $3 \sigma$ confidence). On the other hand, suppose that 10\% of the
% community had malware (a significant fraction), we would expect
% about $400 \pm 45$ alerts, which statistically separates from the
% benign baseline count. 

% However, if there is noise in the community
% structure knowledge or the local detector is more noisy, the fraction
% of nodes that need to have malware can easily rise to 20 - 25 \%,
% which in practice is huge (and thus, not very useful). Thus, count
% alone is of marginal utility if we want to detect malware in its early
% stages.

\noindent \textbf{Space-time Geometry:} The {\em location of alerts}
on the graph is informative -- it is clear that if we observe 100
alerts randomly spread out over the network, then there is not much
cause of worry (likely false positives). However, if we see 100 alerts
all of which are clustered within a few hops of each other (spatial
geometry), then this is much more indicative of a true
malware. Similarly if we first observe an alert at a single node, a
short time later we observe alerts at several of its neighbors, and a
further short time later alerts from their neighbors. This is
evocative of a malware spread (temporal correlation with graph
structure), despite the fact that the total number (count) of alerts
is still very low (and below the false positive uncertainty
threshold).

% Thus, the
% hypothesis testing engine needs to formally incorporate not just
% counts, but also graph space-geometry when making inferences.

\noindent \textbf{Shape of the Distribution:} The third, and perhaps
most subtle effect, is that looking at the {\em inputs to the local
  detectors that send an alert} is informative. That is, instead of
simply counting alerts, {\em we need to exploit the actual
  feature-vectors generating the alerts} (these are eigenvalues if the
feature extraction from the OS trace is based on PCA
\cite{jolliffe2002principal,hearst1998support,scholkopf1998support}). Indeed,
from an information theoretic perspective, this is the right thing to
do because the entropy at the input (feature vector space) to the
(noisy) local detector is greater than that at its output (binary
space).


==> intro/malware-class.tex <==
\subsection{Identifying Malware Classes}

\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.5\textwidth]{synthetic-malware.pdf}
\caption{
Modeling adaptive malware. We 
synthesize
4 information stealers, 2 networked nodes, and 1 compute node, 
in addition to
%The settings represent a small fraction but computationally diverse set of malware behaviors. 
%We also repackage
4 existing malware -- Geinimi, Roidsec, click fraud, and md5 cracker. 
All synthesized malware include the best known obfuscation and 
evasion techniques.
%and use Geinimi which comes repackaged into the MonkeyJump game.
%*Most, but not all, of the workload requires only 100ms.
}
\label{fig:synthetic-malware}
\end{figure}



==> intro/malware-detection.tex <==
\subsubsection{Malware Detection}
\comment{They look at A,B, C on alpha, beta, gamma using blah and saw this. And here is the take away}


Quantitative Study of Accuracy in System Call-Based Malware detection
comparing relative strength of the behavioral detectors
Look at atoms (system calls, syscalls w args, actions (bag of syscalls), actions w args) combined into structures (ngrams, tuples, and bags)
Large scale empirical analysis: approximately 7200 malware samples + 36 benign applications  


Crowdroid:
Analyze the behavior of android applications, providing framework to distinguish between applications that, having the same name and version, behave differently. The aim is to detect anomalously behaving applications. Main contribution is use of crowd sourcing system to obtain system call traces. detected all self written malware with 100\% detection rate. NOTE: IN RELATED WORK Schmidt et al. proposed a solution based on monitoring events occuring on Linux-kernel level. They reviewed Linux based tools for enhancing security, and extracting features such as system calls, modified files, etc. Security tools and mechanisms used in computers are not feasible for applying on smartphones due to the excessive resource consumption and battery depletion. Hence, authors perform whole analysis process on a dedicated remote server. Crowdroid client downloaded from Google app store. Crowdroid monitors syscalls, preprocesses them, and sends them to the centralized server. Server extracts syscall histogram for each execution of each app on a device. Use two cluster k-means as the classifier? Three baseline apps (calculator, countdown, and money converter) written and modified to include malware (NOT SPECIFIED WHAT THIS MALWARE DOES). 60 execution traces collected: 50 Benign + 10 malicious per app. Also tested on Steamy Window + PJApps Malware (100\% detection) and Monkey Jump 2 + HongTouTou Malware (85\% Detection / 3 False Positives). The reason for obtaining a worse detection rate on monkey jump 2 is the simpler nature of the actions performed by the malware. HongTouTou sends information and browses internet while PJApps starts a background application and has more functions programmed. 



A survey on automated dynamic malware-analysis techniques and tools:

Automatic analysis of malware can be performed in two ways. Dynamic analysis refers to techniques that executes a sample and verify the actions this sample performs in practice, while static analysis performs its task without actually executing the sample. The inability to detect unknown threats is an inherent problem of signature based detection techniques. EXTREMELY LONG PAPER, WILL CONTINUE LATER


Andromaly:
Generic and modular framework for detecting malware on Android devices. Host Based. Accomplished by continuously monitoring mobile devices to detect suspicious/abnormal activities using a supervised anomaly detection technique. Light weight application monitors the device for CPU utilization, number of packets sent over Wi-Fi, number of running processes, battery level, average touch pressure, etc. After collection and preprocessing, the system metrics are sent for analysis by various detection units, namely processors, each employing its own expertise to detect malicious behaviour and generate a threat assessment (TA) accordingly. the pending TAs are weighted to produce an integrated alert. The weighting process is per threat type (worms, torgans, etc all have different weights). Weighting process includes a smoothing phase to avoid instantaneous false alarms. Evaluated k-Means, Logistic Regression, Histograms, Decision Tree, Bayesian Networks, and Naive Bayes as classifiers. (MICHAEL NOTE, WTF only a few of these are true classifiers). Used the filter approach for feature selection due to its fast execution time and generalization ability. Under the Filter approach, an objective function evaluates features by their information content and estimates their expected contribution to the classification task. Three feature selection methods were applied: Chi-square, Fisher Score, Information Gain. All 3 follow the Feature Ranking approach. Ranked 88 different features. Developed 4 malicious applications that perform DoS attacks and information theft attacks. First, a Tip Calculator malicious application to unobtrusively perform a DoS attack. When a user clicks the calculate button, the application starts a background service that waits for some time then launches several hundereds of CPU-consuming threads. Schedule SMS, an app to send delayed SMS messages to people. in addition to these malicious apps, 20 benign games and 20 benign tool apps were used. 10\% Overhead when running malware detector at 5s sampling intervals. Best case results changed per experiment with TP/FP ranging from 0.999/0.00 to 0.853/0.162. At time of experiment, no known android malware existed. Second limitation is in small variety of malware applications used.


A Layered Architecture for Detecting Malicious Behaviors:
Build representations of these high-level actions (For example bot actions include proxying, keystroke logging, data leaking, and program download and execute) hierachically, taking care to identify only the essential components of each action. Lowest level even in behavioral specifications are system call invocations. The difference between the low level events and the high level aggregate effect of those events is reffered to as the \emph{semantic gap}. Contributions include a behavior-specification language, a detector for high level actions including distinguishing malicious execution of high-level behaviors from benign. A behavior graph is a directed graph of the form that is adapted from and extends AND/OR graphs. A behavior graph may have AND-edge set and OR-edge sets specifying requirements for actions. Annilhilator nodes are used to represent the destruction of an object or event. replicators duplicate objects. All graphs in this paper were developed manually and iteratively through domain knowledge. Implemented on Qemu emulators. Tainting overhead is 7x-23x wall clock.


Synthesizing Near-Optimal Malware Specifications from Suspicious Behaviors:
This technique, based on graph mining and concept analysis, scales to large classes of programs due to probabilistic sampling of the specification space. HOLMES can synthesize discriminative specifications that accurately distinguish between programs, sustaining an 86\% detection rate on new, unknown malware, with 0 false positives. Behavior based techniques are promising because it is harder for an attacker to radically change the behavior of a malware than to morph its syntactic structure. Constructing behavioral specifications that have a low false positive rate and at the same time are general enough to detect variants of malware is a major challenge. An automatic technique for building these specifications is desirable, both to reduce the AV vendors' response time to new threats and to guarantee precise behavioral specifications. Given a set of \emph{behavior graphs} that describe the semantics exhibited by malicious and benign applications, the graph mining operation extracts \emph{significant behaviors} that can be used to distinguish the malware from the benignware. Wish to find a set of behavioral specifications that describe a given set of programs (the positive set) but not any program  in the second set (the negative set). The first step of the behavior mining algorithm extracts the portions of the dependence graphs of programs from the positive set that correspond to behavior that is significant to the programs intent. I.e. find the subgraphs that give the maximum contrast between the positive and negative sets. (Note mining algorithm determines the notion of significance). Discriminative specification algorithm can guarantee that specifications are optimal with respect to the true and false positive rates over a target sample distribution. Use simulated annealing, probabilistic sampling technique, to efficiently search for a subset of clusters that can be used to construct a close approximation to the optimal specification. Used real Windows malware samples and ran in Qemu. Real world benign apps (putty, FileZilla, Skype, Visual Studio, etc). Able to detect unknown malware with 86.56 percent TP and 0 percent FP. Issue: Can take a while to extract behaviors and these dependence graphs can be big. 


pBMDS: A Behavior-based Malware Detection System for Cellphone Devices:

pBMDS adopts probabilistic approach to malware detection by correlating user inputs with system calls to detect anomalous activities. Leverages HMMS to learn application and user behaviours from two major aspects: process state transitions and user operational patterns. Consider malware such as Commwarrior adopting MMS/SMS and/or Bluetooth as its major infection vector, scanning contacts, randomly choosing some contacts and sending malicious messages to these new victims. Authors assume that malware always launch attacks from the application software (i.e. cannot break the kernel). Once a process deviates from its expected normal behavior(reflected through GUI interactions) to a certain degree, it is considered suspicious and teh access to the system resources should be denied. After learning the user operational patterns and the state transition rules, the engine encodes the learning result by hashing it to the kernel, where it can be safely saved as a user profile. To test whether a running process is malware or a compromised by malware, the run-time detection engine authenticates at key system call points. Runs on Qtopia, a linux based smart phone. After sanitizing the user inputs the next step is to generate a behavior graph which reflects the intermediate process states towards each key system call.


Automated Classification and Analysis of Internet Malware:
The signatures used by IDS and AV often focus on a specific exploit behavior, an approach increasingly complicated by the emergence of multi-vector attacks. As a result, IDS and AV products characterize malware in ways that are incosistent across products, incomplete across malware, and that fail to be consise in their semantics. The reduced collection of user visible system state changes (files r/w, processes created) in a virtualized enviornment is used to create a fingerprint of the malware's behavior. AV systems rarely use dhte exact same labels for a threat, and users of these systems have come to expect simple naming differences. Three key design goals of a label ing system, Consistency, Completeness, and Conciseness. Existing AV solutions fail to meet these metrics. To address these limitations, the authors propose an approach based on the actual execution of the malware samples and observation of their persistent state chagens. Individual system calls may be at a level that is too low for abstacting semantically meaningful information: a higher level abstraction is needed to effectively describe the behavior of malware. State changes are at a higher level than individual syscalls and the avoid many common obfuscation techniques that foil static analysis and low-level signatures. Authors approach to generating meaningful labels is achieved through clustering of the behavioral fingerprints. Initial naive approach to defining similarity was based on the concept of edit distance. Two drawbacks to this approach, it overemphasizes size and behavioral polymorphism (e.g random file names). Instead used normalized compression distance. To combine various pieces of malware based on their similarity, authors constuct a tree structure based on the well-known hierachical clustering algorithm. To extract meaningful groups, the authors adopt an \emph{inconsitency} measure that computes the difference in magnitude between distances of clusters so the tree can be cut into distinct clusters. Evaluate on large and small datasets taken from 2006-2007 including 3698 and 893 unique MD5s respectively. Algorithm created 403 clusters from the 3698 individual malware.  


A Semantics-Based approach to malware detection:
This paper takes the position that the key to malware identification lies in their semantics. It proposes a semantics based framework for reasoning about malware detectors and proving properties such as soundness and completeness of these detectors. Goal of this paper is to provide a formal semantics-based framework that can be used by security researchers to reason about and evaluate the resilience of malware detectors to various kinds of obfuscation transformations. 


DroidMat: Android Malware Detection through Manifest and API Calls Tracing: LOOK AT THEIR RELATED WORK SECTION
Authors propose a static feature-based Android malware detector. Static information includes permissions, deployment of components, Intent messages passing and API calls for characterizing the android applications behavior. Uses k-Means to enhance the malware modeling capability and uses SVD on the low rank approx to determine the number of clusters. Finally, uses kNN algorithm to classify the app as benign or malicious. Dyanamic features often used in literature include logged behavior sequences, system calls, tainting and control flow, and power consumption. Static features used in literature include requested permissions, imported package, API calls, instruction (opcode), data flow, and control flow. Use k-Means and EM in functional behavior recognition. Use spectral analysis to find top singular values covering 95\% of spectral energy. 238 malware samples from 34 malware families collected from Contagio mobile. 50 Benign applications from 30 categories on the Google Play store verified benign using VirusTotal. Accuracy is 97\% with 87\% Recall rate and 96\% Precision.


Semantics Aware Malware Detection:


 Static Analysis?
Authors propose RiskRanker, a scalable automated system to analyze wheter a particular app exhibits dangerous behavior (e.g. launching a rot exploit or sending background SMS). Able to examine 118,318 apps from various Android markets in less than 4 days. Of these, successfully uncovered 718 malware samples in 29 families; 322 of which are zero-day (in 11 families). This is a proactive scheme to spot zero-day Android malware by scalably and accurately sifiting through a large number of untrusted apps without relying on malware specimin. Divide potential risk into high-risk, medium-risk, and low-risk. High risk apps can compromise the phone integrity without authorization, medium risk apps do not exploit software vulnerabilities but can cause users finacial loss/disclose sensitive info. low risk apps may collect device specific, or generic, readily available personal info. For high risk, first scan apps for native code, those with native code are scanned for vulnerability signatures. For medium risk, use symbolic execution to determine which callbacks result in a call to a method of interest. Our first-order analysis modules are mainly designed to handle non-obfuscated apps and may fall short for stealthy malware that intensively encrypts or dynamically changes its payload. To mitigate these weaknesses, we accordingly develop second-order analysis modules to collect and corre-
late various signs or patterns of behavior common among malware yet not among legitimate apps. To evaluate false negatives, authors downloaded 12 malware samples from contagio dump to use as ground truth. System fails to detect social engineering attacks like FakeNetflix. Also fails to detect BatteryDoctor, Gone60, and TapSnake spyware that collect personal info. Also failed to detect ADRD click fraud app. The second reason for failure is taht missed samples do not share the same walicious payload as others in the same family. Finally, some apps are missed because they are guilty by association (e.g. droppers).  


Behavioral Detection of Malware on Mobile Handsets:

Novel behavioral based detector where normal behavior learned from classifier based on SVMs. Also find that the time and resource overheads of constructing the behavior signatures from low level api calls are acceptably low for their deployment on mobile devices. At the time able to detect current mobile viruses and worms with 96\% accuracy. Run on Symbian OS using malware strains gathered from 25 distinct families. Authors reconstruct higher level behavior signatures from lower level API calls. Train SVMs with both normal and malicious behaviors so that partial signatures for malicious behavior can be classified correctly. Behavior signatures are best specified using temporal logic instead of classical propositional logic. Monitor a subset of symbian API calls using temporal logic of causal knowledge (temporal logic TLCK). Authors manually generated propositional variables and TLCK operators to create the behavior signatures for each family. Plan on exploring automated feature extraction methods. Construct the behavior signatures of a program at runtime by generating, pruning, and aggregating, dependency graphs. Use Gaussian radial basis as kernel method in SVM.

% http://ieeexplore.ieee.org/xpls/abs_all.jsp?arnumber=6170530&tag=1

==> intro/malware-propagation.tex <==
% Malware propagation
\subsection{Network Malware Propagation}
\label{sec:malware-prop}

% \comment{
% Spatial-Temporal Modeling of Malware Propagation in Networks:

% Due to huge potential damages that may be caused by malware, researchers have proposed many models to describe the dynamic process of malware propagation. The goals of the these propagation models can be classified into the following categories: (1) gain a deep understanding of the propagation mechanisms of malware. (2) predict the scale of the malware outbreak before it actually occurs; (3) evaluate how network provisioning impacts the propagation and how propagation impacts the network; (4) characterize the infection dynamics of malware; and (5) design countermeasures to restrain malware propagation.

% Infection vectors:
% - SMS/MMS:  ComWar worm browses hosts phonebook then spreads via SMS/MMS

% - Bluetooth\cite{Yan4268196,Yan4624266,rhodes2008,carettoni2007}: Device to device malware spreading: Limited attack vector because devices generally not in discovery mode, discovery period is limited, and file transfer requires user confirmation. 

% - Internet Access: Similar to PC enviornment

% - Compromised USB: for example if the programs used to synchronize smartphones were compromised.

% A representative unified and integrated propagation model remains unknown to the cyber security community. 
% Yan and Eidenbenz built an analytical model to study the spread of Bluetooth worms\cite{Yan4268196,Yan4624266}. They describe the impact of mobility patterns by investigating input parameters, such as average node degree, average node meeting rate, and link duration distribution.

% Rhodes and Nekovee \cite{rhodes2008} invesitaged the effect of population characteristics and device behavior on the outbreak dynamics of Bluetooth worms using SIP model. They assumed there is a single infected device capable of infecting any nearby device with probability p. Did not characterize the spatial-temporal characteristics of the propagation dynamics of Bluetooth worms, and also did not consider the impact of individual difference on the propagation dynamics of different worms. 

% (Superimposed graphs) Gao and Liu\cite{Gao2011,Gao2013} proposed a two layer model to simulate the propagation process of Bluetooth-based and SMS-based viruses. They modeled bluetooth propagation as a geographical overlay on a 2-dimensional grid. They modeled SMS-based virus propagation as a logical contacts graph where each node is a cell phone and the links are derived from address books. This evaluates the effects of human operations on SMS-based virus propagation and the effects of human mobility on geographic networks.

% Ramachandran and Sikdar\cite{Ramachandran2006,Ramachandran2007} presented analytical models to explore the impact of spreading mechanisms such as downloads from the Internet or P2P networks, WLAN and infrared interfaces and through MMS or SMS messages on the dynamics of malware propagation in smartphone networks. 

% most of the discussed models do not consider all possible input parameters. For example, most models have neither considered the impact of individual differences on malware propagation, nor considered the impact of human behavior on malware propagation. Nor did any describe the impact of random mobility on smartphone users. 

% Peng et al. \cite{Peng2013}
% }


% \comment{
% Mickens and Noble\cite{Mickens2005} proposed a probabilistic queuing framework to model the propagation of mobile malware over short-range wireless interfaces. This model emphasizes node mobility, a key factor in the non-homogeniety of near-proximity based mobile networks, as the node speed effects the steady state infection level of the network. \comment{This model accounted for movement and traffic patterns over various time durations(Not seen in previous analytical models)}

% Yan and Eidenbenz\cite{Yan4268196,Yan4624266} built an analytical model to study Bluetooth worm propagation. According to this model, the impact of mobility patterns on Bluetooth worm propagation can be investigated by introducing input parameters (e.g. link duration distribution, average node meeting rate, and average node degree). 

% Rhodes and Nekovee \cite{rhodes2008} invesitaged the effect of population characteristics and device behavior on the outbreak dynamics of Bluetooth worms using a susceptible-infected-removed (SIR) model. They assumed there is a single infected device capable of infecting any nearby device with probability p. Infected devices are removed, for example, if they become innoculated by an exploit patch. 

% Martin et al. \cite{Martin2010} predicted the spread of mobile platform viruses using the susceptible-infected-susceptible (SIS) model from mathematical epidemiology. In this model a node may be cured of infection but is still susceptible to a new infection. 


% Peng and Wang \cite{Peng2011, Peng2013} proposed a worm propagation modeling scheme (WPM) which simulates the dynamics of worm propagation process from a single node to the entire network using 2D cellular automata. This model takes into consideration the spread of of infected nodes in a network and offers a resistance factor to the susceptible nodes. 
% }
%\subsubsection{Proximity Attacks}%: e.g. modeling Bluetooth worms


To evaluate our GD algorithms, we use a grid, a random graph, and a
social network to connect the LDs. Indeed, there has much recent study
on network based malware/virus spread including propagation models
(e.g. SI, SIR, SIS), graph properties, and simulation/empirical
results
\cite{Mickens2005,Yan4268196,badusb,Fan2010ANSONAM,Yan4624266,suetal06:blueworm,Mickens2005,Cheng2007,wang09:spreading,kleinberg07:wlessepi,massganesh05:epidemics,kepwhite91:viruses}.
We highlight the work in \cite{massganesh05:epidemics}, where the
effects of graph structure on spread dynamics was characterized for a
variety of graphs. The spread can occur in various ways, e.g. over
geographical networks, online networks, call contact graphs,
proximity, etc. Further, the spread can be explicit (i.e., over the
contact graph itself) or implicit (i.e., the word-of-mouth contact
graph popularizes a malicious app, but the actual download is from a
app store).

We abstract these into three archetypical graphs: grid, random and
social. The grid graph, with small cycles and large diameter, captures
proximal networks for the spread (e.g. word-of-mouth, USB drives,
bluetooth). The random graph and social graph capture online networks
which have small degree but also a small diameter (i.e. things spread
rapidly). Phone contact graphs, Facebook graph, and email contact
graphs are illustrative of this class.


%models for how malware propagates across each LD-graph. 

% Malware often spreads through short-range wireless interfaces like
% Bluetooth~\cite{Mickens2005,Yan4268196,Yan4624266} or physical devices such as
% malicious USB drives~\cite{badusb}. Such proximity-based malware propagation
% can be modeled using a grid network of LDs.  In addition, we also study random
% graphs which are widely used as crude first-order model of networks with low
% diameter and small degree.

% Malware also spreads over contact graphs. For instance, Fan et al.
% \cite{Fan2010ANSONAM} discuss a model of computer viruses that transmit through
% Facebook and email, finding that the worm spreads through the contact graph and
% that Facebook worms spread faster than email worms. Further, Xin et al.
% \cite{Xin2009} examined the propagation of worms through a lens of game theory,
% concluding that camouflaged worms play better than naive worm and consequently
% propagate faster. 



%Much of the early research in modeling mobile malware propagation was
%spurred on by the worms Commwarrior and Cabir. 

%The Cabir worm propagated over Bluetooth, and CommWarrior over both Bluetooth
%and SMS/MMS \comment{(it picked contacts at random to send to)}.  For example,
%Mickens and Noble\cite{Mickens2005} proposed a probabilistic queuing framework
%to model the propagation of mobile malware over short-range wireless
%interfaces. Their model emphasizes node mobility, and determined it to be a key
%factor in the non-homogeneity of near-proximity based mobile networks, as the
%node speed affects the steady state infection level of the network. This model
%accounted for movement and traffic patterns over various time durations, a
%contribution not seen in previous analytical models.  Similarly, Yan and
%Eidenbenz\cite{Yan4268196,Yan4624266} continued studying Bluetooth worm
%propagation, determining that the impact of mobility patterns on Bluetooth worm
%propagation can be investigated by introducing input parameters to the model
%(e.g. link duration distribution, average node meeting rate, and average node
%degree).

% \ignore{
% Malware propagation models also borrow from mathematical epidemiology.  Rhodes
% and Nekovee \cite{rhodes2008} investigate the effect of population
% characteristics and device behavior on the outbreak dynamics of Bluetooth worms
% using a susceptible-infected-removed (SIR) model. They assumed there is a
% single infected device capable of infecting any nearby device with probability
% p, but where infected devices can be inoculated by a security patch. Later,
% Martin et al. \cite{Martin2010} described the spread of mobile malware using a
% susceptible-infected-susceptible (SIS) model.  In this model a node may be
% cured of infection but is still susceptible to a new infection.  Peng and Wang
% \cite{Peng2011, Peng2013} proposed a worm propagation modeling scheme (WPM)
% which simulates the dynamics of worm propagation process from a single node to
% the entire network using 2D cellular automata. 
% }

%This model takes
%into consideration the spread of of infected nodes in a network and offers a
%resistance factor to the susceptible nodes.



%Unlike proximity-based infections, malware that propagates through the internet
%has the potential to do significantly more damage\cite{morris-worm, storm-worm, conficker-worm}\comment{\todo{CITE} \michael{Morris
%Worm, Storm Worm, Conficker Worm}

% https://tools.ietf.org/html/rfc1135 Morris Worm,
% https://www.f-secure.com/v-descs/small_dam.shtml Storm Worm,
% http://www.microsoft.com/security/portal/threat/encyclopedia/entry.aspx?Name=Worm:Win32/Conficker.E#tab=2
% Conficker} 

%[Morris Worm, Storm Worm, Conficker]} and smartphones offer a mobile platform
%for such worms 
%Previous work models the spread of these internet worm through


% Ultimately, mobile platforms suffer from a multi-vector attack scenario. As
% such, researchers have proposed hybrid propagation proximity-based and
% internet-based models. In general, this is captured via Bluetooth and SMS/MMS
% models. Cheng et al.~\cite{Cheng2011MalProp} proposed the first hybrid
% analytical model based on the propagation of the CommWarrior worm, measuring
% the speed and severity of its propagation.  Ramachandran and
% Sikdar~\cite{Ramachandran2006,Ramachandran2007} explored the impact of
% spreading mechanisms such as downloads from the Internet and P2P networks,
% infrared interfaces, and through MMS and SMS on the dynamics of malware
% propagation in smartphone networks. Xia et al.~\cite{Xia2008} further
% considered the situation where an infected device may be in a dormant state.
% Fan \cite{Fan2010:5601326} built a hybrid model based on preventative immunity,
% and virus mutation that takes mobility of the actors into account. Gao and
% Liu\cite{Gao2011,Gao2013} proposed a two-layer hybrid model using superimposed
% graphs. They model bluetooth propagation as a geographical overlay on a
% two-dimensional grid and  SMS-based propagation as a logical contacts graph
% where each node is a cell phone and the links are derived from address books.
% Therefore, their work considers both the effects of human operations on
% SMS-based propagation and the effects of human mobility on geographic networks.






==> intro/related-work.tex <==
% \subsection{Related Work}

\comment{
\mohit{from proposal}
Inference on networks has seen a lot of
interest recently, with research on determining epidemic source aka rumor
source) \cite{infectionsource,zash11,karam13,luo12,luo13,zhuyin}, learning
network structure from observations \cite{gomez2012,netrapalli12}, and
inferring for causation (work by PIs)
\cite{milling12,allerton2012,mobihoc2013,meirom14}. Beyond the epidemic
context, statistical models for parameter learning
\cite{dene05a,dene05b,streftaris02,demiris05b,bane04} and anomaly learning
\cite{acd08,acd11} have seen much progress over the last decade. Our approach
-- dynamic learning from weak signals for reducing false positives/negatives
using the network -- is a new direction. Tangentially related are works with
active detection techniques where one considers optimal sensor placement for
epidemic detection, e.g., \cite{LeskovecKDD2007}.
%
From a systems perspective, such network based approaches have been studied in
the context of collaborative IDS \cite{dash06,seurat,IDS-survey15} (also see
related works in Section~\ref{sec:arch}).  Most relevant is \cite{dash06} where
the authors use a variety of count methods (analysis of the time series of
cumulative alert counts) at a global level by aggregating all the local
detector counts. As discussed earlier, the space-time geometry emerging from
the community structure and shape distributions of true and false positives
provide a more nuanced lens for detecting zero-day exploits.
% Thus, the key innovation in our approach is that we use the fine-grained
% community space-time structure as a lens to filter and bias alert samples --
As we will see in Figure~\ref{fig:eigen} and Question~4, these insights provide
a powerful boost for early stage malware detection.
}

\input{intro/behavioral-analysis}
\input{intro/cids}
\input{intro/malware-propagation}


==> intro/threat.tex <==
\subsection{Threat Model and Assumptions}
\label{sec:threat}

%Mobile app ecosystems are complex and we minimally consider a system
%with six principals -- users, benign and malware app developers,
%mobile platform providers, hardware manufacturers, malware analysts,
%and finally \sysname itself.  

We assume that a large fraction of our
users and developers are benign and can provide data to build robust
models.  \sysname is thus best suited for early stage malware
detection -- if the majority of devices are compromised, behavioral
analysis is useless.  Malware developers are untrusted and can exploit
apps, the underlying operating system and hardware, and even trick
users into installing overprivileged apps.  The end result is that
malware turns a fraction of the devices on a network into active
adversaries that attempt to evade detection while executing malicious
payloads.
%
%
The remaining principals function similar to traditional Collaborative IDSs.
Platform providers like Google and Samsung are trusted and can open up
important operating system and hardware-level signals for malware detection.
We trust hardware manufacturers like Intel and Qualcomm to implement their
instruction sets without hardware backdoors.  Malware analysts are trusted but
only to provide malware detection results and are not trusted to view or infer
users' private data.  Finally, we trust \sysname as a platform to collect,
seal, and declassify user data.


==> notes/graph-size.tex <==
% Graph Size

I am not convinced that we need to process any graph larger than 15k nodes to prove our point. Consider the UT computer network. Here, machines are probably distributed between \textit{buildings} or \textit{departments} with reasonable density. Consequently, we can consider strong subgraphs as a partition of the overall graph structure. Each subgraph contains some notion of a community structure and the connectivity between subgraphs is extremely low (potentially disjoint) therefore we can process each subgraph independently and aggregate at a later time. This should reduce processing time dramatically at the cost of adding noise to the time to detection.   


==> previous_submissions.tex <==
\begin{table}[htb]	
	\resizebox{\columnwidth}{!}{%
    \begin{tabular}{| l | l | l | l |}
    \hline
    Conference & Score 1 & Score 2 & Score 3 \\ \hline
    CCS'16 & 5 (accept) & 3 (weak reject) & 3 (weak reject) \\
    NDSS'16 & 3 (weak accept) & 3 (weak accept) & 2 (weak reject) \\ \hline
    \end{tabular}
    }
    \label{tbl:previous_submissions}
   	\caption{The paper was submitted to CCS'16 and NDSS'16.}
\end{table}


\noindent{\bf CCS'16.} 
The key complaint was that the paper needed to formally
describe the Shape GD algorithm, and to explain how neighborhoods
can be defined by an analyst. {\bf Improvements:}

\begin{enumerate}

\item Added formal description of Shape GD's algorithm.

\item Clarified how neighborhoods can be defined based on attack vectors.
(More generally, based on either information flow sources
or sinks of an enterprise system.)

\item Added a deployment section and tied it closely with questions
answered in the evaluation.

\item Added overhead section.

\end{enumerate}


\noindent{\bf NDSS'16.} The key complaint was to differentiate Shape GD from
clustering GDs instead of only (ensemble etc) based Count GDs. {\bf
Improvements:} 

\begin{enumerate}

\item Quantified the best known clustering algorithm's performance on our
dataset and explained why clustering and similar methods are fundamentally
limited against high-dimensional data.  Neighborhoods overcome these
limitations -- since they capture transient correlations that impose a
low-dimensional structure on the raw data.

\item Updated theoretical description of the algorithm.

\item Implemented Shape GD within a real-world SIEM infrastructure (at a Fortune-500
company) (see Appendix B). We identified a set of new challenges:
extremely high-dimensional and sparse data, delayed records, uniquely identifying
devices and users from log records -- addressing all these challenges is in our
roadmap and deserves an entire paper. This paper focuses on a homogeneous GD
as deployed by users of (e.g.) {\tt osquery} and studied in a large majority
of prior work (E.g., we replicate the malware and benignware datasets from
BareCloud in Usenix 2014 and use real datacenter traces from Yahoo).

\end{enumerate}


==> results.tex <==
%\input{results/intro_results}

%\subsection{Local Detectors and Feature Extraction algorithms}
%\label{sec:LDs}
%\input{results/LDs}

\todo{

Assume:
\begin{itemize}
\item community
\item neighborhood. applied to phishing and waterhole.
\item filtering
\item shape (idea) --> wasserstein distance (metric).
\end{itemize}

Why each subsection?
\begin{itemize}
\item Top-level goal: Early detection as malware infects a neighborhood.
How early? We proceeed in three steps.

\item Step 1: 
How well can GD distinguish between {\em purely} benign v. malicious
neighborhoods? This is a baseline test for shape-based GD. In the
next two subsections, we will use shape-GD to classify neighborhoods 
with early-stage infections from benign neighborhoods -- i.e., when
malicious neighborhood has {\em a mix of benign and malware FVs}.
%-- i.e., shape-GD has to
%distinguish a mix of malicious and benign nodes.

\item Step 2: 
Phishing: how {\em quickly} can shape-GD detect malware if it spreads through
a few malicious emails among many benign emails in a enterprise network?

\item Step 3:
Waterhole: how {\em quickly} can shape-GD detect malware if it spreads
through a few malicious servers that compromise clients that visit the
malicious servers?

\end{itemize}



How + Results.
\begin{itemize}

\item [Ref Section 4] Each nbd has a score -- i.e., 
Wasserstein distance metric -- and in Fig X, we will plot the histogram
of scores from N benign nbds v. N malicious nbds.

Explanation: Perfect separation at 15k FV/nbd. 
But partial overlap of benign and malicious histograms may be ok -- this 
creates GD FPs. 

\item Phishing. Early detection using shape-only: shape works at 22 [Fig X].
On the other hand, small errors in count lead to large errors in 
time to detection [Fig Y]. In Fig Z, we show that shape + NF improves
shape-only by 4X

\end{itemize}
}






We now report the main results of our computations. Ultimately our
goal is to demonstrate that our overall LD + GD framework is effective
and hence presents a new paradigm for early detection of new malware
epidemics. In addition, we present a host of ancillary or intermediate
results, that demonstrate the conceptual underpinnings of this
paper. We present results on our local detectors. We test the
effectiveness and robustness of the shape-based detection that
underlies our GI engine, and compare to count-based algorithms. We
expand on Figure~\ref{fig:intro-histogram} to show what at some level
is the cornerstone technical piece of our approach: the fact that the
conditional distributions of false positives and true positives are
well separated in the right metric -- we present several more
supporting results.

\subsection{Local Detectors are Noisy}

In Section \ref{sec:exp-set}, we describe the local detector we finally select.
We provide here some interesting aspects of the detector we use in our overall
framework. The LD results in Figure~\ref{fig:ROC} show three interesting
trends. First,  Random Forest outperforms all other classifiers.  2-class SVM
and Decision Tree algorithm are close to but lower than Random Forest in terms
of detection accuracy. Second, the \intbasis LD algorithm leads to poor
detection results across all ML classifiers. The Histogram and n-gram FE
algorithms are almost identical in terms of detection accuracy -- hence we
favor histogram FE algorithm over n-grams because n-gram models are
computationally expensive to run on client devices.

The key result from this study is that we use Random Forest with a
histogram-based FE algorithm as a representative LD. In our choice, the
assumption is implicit that the best performing LD will yield the best GD. This
is plausible because if we have no side information about the new malware we
are hoping to detect (and indeed, we assume this is the case), any degraded LD
performance is simply noise that we should not expect to do anything but
deteriorate the performance of any global inference engine using its output as
input. A related point to make is that we believe our main contributions in our
Global Inference Engine framework, begin where the LD leaves off. That is to
say, we expect that a better LD could be easily integrated into our framework,
and we believe it would only lead to improved results.

\subsection{True from False Positives: The Power of Shape}
\label{sec:pure_shape}
\input{results/pure_shape}

\subsection{Global Inference Engine: ROC}
\label{sec:GD_ROC}
\input{results/GD_ROC}

\subsection{Shape vs Count without censoring}
\label{sec:shape_vs_count}
\input{results/shape_vs_count}

%\subsection{Number Of Bins}
%\label{sec:bin_number}
%\input{results/bin_number}

%\subsection{Censoring algorithm.}
%\label{sec:censoring}
%\input{results/censoring}

\subsection{Censoring Algorithm: Neighborhood Filter}
\label{sec:censoring}
\input{results/detection_threshold_vs_censoring_threshold}

\subsection{Detection Threshold Scales As Log(n)}
\label{sec:ttd_as_log_n}
\input{results/log_n}

\subsection{Detection threshold vs percentile}
\label{sec:detection_threshold}
\input{results/detection_threshold_vs_percentile}

%\subsection{Learning the basis.}
%\label{sec:basis_learning}
%\input{results/basis_learning}

%\subsection{Robustness To Polluted Training Data}
%\label{sec:robustness_polluted_training_data}
%\input{results/robustness_polluted_training_data}

%\subsection{Robustness To Compromised Local Detectors}
%\label{sec:robustness_compromised_LDs}
%\input{results/robustness_compromised_LDs}

%\subsection{Protecting Multiple Versions Of An App [Michael]}
%\label{sec:multiple_app_versions}
%\input{results/multiple_app_versions}
%
%\subsection{Android Monkey vs Real User Input [Michael] (Drop it)}
%\label{sec:monkey_vs_real_user}
%\input{results/monkey_vs_real_user}
%
%\subsection{Cause Analysis. Supervised Learning???}
%\label{sec:cause_analysis}
%\input{results/cause_analysis_intuitive_basis}


==> results/GD_ROC.tex <==
\begin{figure*}[t]
  \begin{minipage}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/GD_ROC/GD_ROC_Random_Forest.pdf}\par
    \subcaption{Random Forest}
\label{fig:GD_ROC_RF}
  \end{minipage}
  \begin{minipage}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/GD_ROC/GD_ROC_2_class_SVM.pdf}\par
    \subcaption{Two-Class SVM}
\label{fig:GD_ROC_SVM}
  \end{minipage}
  \begin{minipage}[t]{0.33\linewidth}
    \centering
    \includegraphics[width=\textwidth]{figs/GD_ROC/GD_ROC_AdaBoost_Decision_Trees.pdf}\par
    \subcaption{Boosted Decision Trees}
\label{fig:GD_ROC_BOOSTED_DTs}
  \end{minipage}
  \caption{Shape GD's ROC curves. In most of the cases we consider,
      Shape GD perfectly separates false and true positives -- this is shown by
      black  step-wise curves. It is worth noting that histogram separation
      depends on an LD that is used -- GD and LD should be co-designed.}
  

\label{fig:GD_ROC}
\end{figure*}

For most apps, Shape GD achieves perfect separation of false and true positive
distributions of FVs (Figure~\ref{fig:histogram}); sometimes, however, we observe in our results that the conditional distributions display a slight overlap. In those cases, the robustness threshold
$\gamma$ (see Section~\ref{sec:algo_description}) should be carefully chosen to avoid
global false positives, i.e., to avoid mislabeling communities as infected. In this section, we explore and quantify more carefully, our ability to separate true and false positives, i.e., we quantify the performance of Shape GD. We do this via ROC curves. ROC curves provide a standard method for analyzing the trade-off between global FPs and TPs.% before choosing a particular $\gamma$.

%As discussed earlier, 
%Shape GD makes a decision on labeling incoming FVs as malicious or benign based
%on the hypothesis test parameterized by the robustness threshold $\gamma$ (Section\todo). In our implementation, we set $\gamma$ 
%based on the shape of FP and TP distributions (Figure~\ref{fig:histogram}),
%%When choosing a particular $\gamma$, we try 
%with the goal of minimizing the global false positive rate.

To build an ROC curve, 
%instead of choosing a concrete value of $\gamma$, 
we sweep the entire range of values that $\gamma$ can take. For each such
value, we record a corresponding GD true and false positive rate
%And then by combining them, we 
to obtain an ROC curve for the app. 
%We have plotted ROC curves for
Figure~\ref{fig:GD_ROC} shows the Shape GD's 
ROC curves for all apps in our experiment.
%Shape GD and all the apps from our corpus 

%As expected, ROC plot shows the trade-off between global false and true
%positives. 

The most interesting part of this ROC plot is that half of the apps' ROC curves
-- the black line -- have a step-shape because Shape GD achieves flawless
separation between local FPs and TPs. This follows from the TP v. FP histograms
in Figure~\ref{fig:histogram}.
%From analysis of ROC plot, we see that Shape GD demonstrates ideal accuracy
%when running on the following 
The five apps with perfect ROC curve are AVG, Buzzfeed, All Recipes, Wikipedia, and Zedge.  Three
other apps -- Walmart, Bible, eBay -- have slightly overlapping distributions
of local false and true positives, hence the corresponding ROC curves deviate
from the step-shape. And finally the last two apps -- Yelp and Html5 -- do not
have separable distributions of TPs and FPs when processed by our Shape GD,
i.e., global detection may lead to community-level misclassification. 

%We exclude those apps from the further consideration.
GD's performance depends on a choice of LD (Figure \ref{fig:GD_ROC}). When
using Random Forest as LD, GD does not work for Yelp and HTML5. However, if we consider
2-class SVM, then GD is able to process Yelp. Similarly, if 
we switch to Boosted Decision
Trees LD, then GD can handle both apps, but it does not work well for Buzzfeed.
Thus, LD and GD should co-designed.

In summary, 
%when choosing a concrete value for 
setting the robustness $\gamma$, i.e., the GD's false positive rate, 
to 10\%, yields a true positive rate close to 100\% for 
%accurate results and does not sacrifice detection rate because 
all apps except Yelp and Html5. In comparison, the constituent LD
only yields a detection rate of 80\% for a false positive rate of 10\% (Figure~\ref{fig:ROC}). And again, for the majority of the apps we tested, GD's (global) false positive rate is reduced to effectively 0\%, while achieving a detection rate of 100\%. 
%\todo{Say what the baseline LD} 
%have global true positive rate higher than 95\%.
%\todo{for what FP rate: zero?}




==> results/basis_learning.tex <==
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/dictionary_learning/dictionary-learning.pdf}\par
\caption{\textit{(Learning the types of system calls) How long does it take to observe all types of system calls that get issued over all program execution?}}
\label{fig:dictionary_learning}
\end{figure}

In this experiment we try to learn how long it takes to learn all types of system calls that are issued by a program. We randomly permute the set of benign FVs 10 times and compute 10 curves, each of them shows how long it takes to learn the set of system calls that are actively used by a program. After that we average all of the curves and plot the average.

HTML5, Yelp and All Recipes converge fast -- they require to observe fewer than 1000 FVs to be able to deduce more than 94\% of system calls that are actively used. Sana Med. App and Wikipedia converge much slower. We need to observe 5000 FVs on average to learn more than 94\% of used system calls.



==> results/bin_number.tex <==
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/number_of_bins.pdf}\par
\caption{\textit{(Shape detector: Effect of binning on the detector's sensitivity.}}
\label{fig:num_of_bins}
\end{figure}

When tuning parameters of our global detector, we noticed that the way we discretisize  the data, i.e. compute \textit{pmf}, is crucial for the overall performance of the global detector.

By analyzing distribution along every principal in the training phase, we notice that distributions usually have very long tails. When we apply standard binning algorithm with uniform bin sizes, we obtain many empty or almost empty bins. The drawback of such straightforward binning is that 1) global detector has to operate high-dimensional pmfs; 2) \sysname is extremely sensitive to any noise due to huge number of low populated bins.

To overcome this issue, we trim the tails of the distribution -- the data below 1th percentile and above 99\% percentile. The trimmed tails are represented as two separate bins of infinite size. The rest of the distribution is covered with a few dozens of bins, whose number is defined based on either "square-root choice" sqrt(n) or Scott's normal reference rule $3.5*sigma/n^0.33$. The Scott's rule calculates different number of bins for each dimension of data. And we choose the maximum number to achieve the highest resolution. For example, in the case of Wikipedia the former rule results in 33 bins and the latter results in 55 bins. In our experiments we do not observe significant difference between these strategies of choosing the number of bins. Thus, we stick to Scott's rule for consistency.

As an alternative solution we tried to apply non-uniform binning, but binning based on either square-root choice or Scott's rule gives better results than non-uniform binning.

Also we swept the parameter space to get a better feeling of whether our binning strategies are reasonable or not~\ref{fig:num_of_bins}. The resolution of the x axis is 10. For every value of the parameter "number of bins", we computed the contamination level of the input data set that triggers global detector. We averaged the results over 10 runs of the experiment. The plot shows that the global detector starts reacting to malware if its level exceeds 8\%. Indirectly, the plot proves that our strategy for choosing the number of bins is adequate because none of the two choices gives advantage over the other one.



==> results/censoring.tex <==
%\begin{figure}[tbp]
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/wiki_vs_censoring_threshold.pdf}\par
%\caption{\textit{(Wikipedia) Detection rate vs censoring threshold.}}
%\label{fig:wiki_vs_censoring_threshold}
%\end{figure}


==> results/detection_threshold_vs_censoring_threshold.tex <==
%Despite the low detection threshold (5-15\% in sec.~\ref{sec:shape_vs_count})
%achieved by Shape GD, large absolute numbers of nodes in a network need to be
%infected before \sysname is able to spot malware. 

To further reduce the time to detection, we apply the Neighborhood Filtering
(NF) algorithm (see Section~\ref{sec:algo_description}) to the baseline Shape GD.
Recall that NF is a neighborhood alert-density dependent censor, i.e., it
considers an alert in the Shape GD only if the number of alerts in
its local space-time neighborhood are above a {\em censoring threshold}. 
%Here we analyze the Shape GD benefits from
%Neighborhood Filtering.
%We have already seen (Figure~\ref{fig:shape_vs_count}) that Shape GD is able to achieve detection rate of 8.8\% (Figure~\ref{fig:shape_vs_count_random}) and 14.4\% (Figure~\ref{fig:shape_vs_count_social}) in a network with random graph topology and in a social network respectively. Its performance is much better in the case of grid topology - 4.6\% (Figure~\ref{fig:shape_vs_count_grid}). Even if these numbers are quite small, the absolute number of infected nodes can be large in big networks.

Intuitively, to eliminate a majority of false positives, the censoring
threshold $\lambda$ should be above the LD's FP rate. To confirm this, we vary the
censoring threshold from 0\% up to 100\% and record the corresponding value of
detection threshold. Figure ~\ref{fig:censoring} shows the results of
this experiment with three types of networks: random, grid
and social network. The horizontal axis shows censoring threshold $\lambda$,
and the vertical axis corresponds to the detection threshold. The robustness
threshold $\gamma$, i.e., the GD's false positive rate, is set to 10\%.
%Whatever topology an underlying network has, 

We find that the optimal range for the censoring
threshold $\lambda$ is between 35\% and 80\% for all three network topologies. 
When $\lambda$ is less than 35\%,
i.e., close to the LD's false positive rate, detection threshold is higher and unstable.
Conversely, if censoring threshold is too high, too many true positives
get filtered out and GD is only able to spot malware in a community when almost
all nodes are infected. 

%If we look how NF affects GD's performance for individual networks, 
We observe that NF improves GD's performance the most for random
networks (detection threshold drops from 10\% down to 3\%) -- this happens due
to the presence of multiple long-range connections between network nodes. Even
though Shape GD worked best for a grid network, NF improves its performance by a 
%spite of demonstrating the best detection results in grid network, Shape GD is
further 5$\times$ (0.6\% from 3\%). For the
social network, detection threshold goes down to 2.2\% from the
original 10\%.

Overall, NF censoring helps to bring detection threshold down by 3-5$\times$ and keeps it under 3\% level for all three networks.


%GD's performance on random network is affected the most by censoring and detection threshold drops from 10\% down to 3\%. One can observe similar trend for social network -- detection rate goes from 9\% down to 2.2\%. GD also benefits when running on a graph with grid topology -- drop from 3\% down to 0.6\%. Thus, censoring helps to bring detection threshold down by 3-5x and keep it under 3\% level for all types of network.

%Detection threshold remains low till reaching 80\% censoring threshold. After that it goes up because censoring algorithm ignores too many malicious neighborhoods, thus GD does not receive any incoming data. Only if a large portion of a network is infected, then GD starts receiving malicious data and is able to label it correctly.

%We choose 50\% censoring threshold for the remaining experiments.


==> results/detection_threshold_vs_percentile.tex <==
Shape GD relies on the hypothesis test (Section~\ref{sec:algo_description}) that
is parametrized by the robustness threshold $\gamma$. 
%For a fixed $\gamma$,
%GD's output has confidence $1-\gamma$. 
Low values of $\gamma$ lead to a low GD false positive rate, but they may also result in low detection thresholds (and thus late malware reporting). We analyze GD's sensitivity to $\gamma$ to balance time to detection and accuracy of GD's output.

We vary the robustness threshold $\gamma$ from 0\% (percentile) up to 50\%
and 
%When $\gamma$ is set to 50\%, GD's output
%is correct with probability 50\% -- it is equivalent to random guess, that's
%why we do not go beyond the value of 50\%. As usual, we repeat the same
experiment with the three types of networks: random, grid, and social network.

Figure~\ref{fig:detect_vs_prctile} plots the detection threshold v. the censoring
threshold -- so that a low value on Y-axis is better. 
If we exclude effect of NF,
detection threshold drops fast -- 36\% vs 12\%, 28\% vs 8.8\%, 11.5\% vs 3.5\%
for random, grid and social networks respectively -- when increasing $\lambda$
from 0\% up to 10\%. With no censoring, 
10\% is a reasonable value for $\lambda$ that
%moves GD's performance to the desirable range, i.e., 
moves detection threshold to
under 12\%.

Neighborhood filtering (NF) (sec.~\ref{sec:censoring}) brings
the curves closer to the horizontal axis and makes them flatter
(Figures\ref{fig:detect_vs_prctile}). However, the left-hand side part of
the curves corresponding to the values of $\gamma < 10\%$ has steep slope. It
is still beneficial to admit 10\% error by setting $\gamma = 10\%$. If
censoring threshold $\lambda = 50\%$, i.e., the third graph on the right, then setting $\gamma$ to 10\% let us
reduce detection threshold to less than 2\% level across all network toplogies
that we consider. It is worth noting that Shape GD's detection threshold in
grid network has very low value of 0.3\%.

Shape GD is mainly governed by two parameters - the censoring threshold
$\lambda$ and the robustness threshold $\gamma$. Based on the analysis of GD's
sensitivity (sec.~\ref{sec:censoring} and sec.~\ref{sec:detection_threshold})
to these parameters $\lambda = 50\%$ and $\gamma = 10\%$ seem to be an optimal
setting that allows Shape GD to identify malware spread at an early stage and
keep high accuracy of GD's detection results.


==> results/intro_results.tex <==
\mikhail{In the the following subsections we walk a reader through the process of
building a network-level malware detector and justify every step. 

First, we start with consideration of a few local detectors (LDs). 
Second, we
address our premise that shape of distribution contains much more information
than a simple aggregation of LDs' outputs. Third, we evaluate the role of
space-time geometry for both shape and count-based detectors. Forth, we
estimate fault-tolerance properties of our system under assumptions that some
LDs and network media may be brought down by an attacker or due to
software/hardware failure. And finally, we bring our attention to the one of
the most crucial problems in malware detection -- "cause analysis". As a result
of the design solutions made at earlier stages, \sysname allows a malware
analyst easily find out high-level malicious behavior. Partially, this is
achieved by using a completely novel technique in the field of computer
security -- dictionary learning.}


==> results/log_n.tex <==
\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/log_n/log_n_all.pdf}\par
\caption{(Wikipedia app) Detection threshold scales as a logarithmic function of network size.}
\label{fig:wiki_vs_censoring_threshold}
\end{figure}


\begin{figure}[tbp]
   \centering
   \includegraphics[width=0.45\textwidth]{figs/detection_threshold_vs_censoring_threshold/combined.pdf}\par
\caption{(Wikipedia app) Detection threshold vs censoring threshold. We analyze the effect of censoring on the detection threshold. Censoring threshold reduces detection threshold if it is above LD's FP rate.}
\label{fig:censoring}
\end{figure}

\begin{figure*}[t]
\begin{minipage}[tbp]{0.3\linewidth}
%   \begin{flushleft}
  \centering
   \includegraphics[width=\textwidth]{figs/detection_threshold_vs_prctile/no_censoring/combined.pdf}\par
   \subcaption{{No censoring}}
   \label{fig:detect_vs_prctile_no_censoring}
%   \end{flushleft}
\end{minipage}
%\hfill
\begin{minipage}[tbp]{0.3\linewidth}
%   \begin{flushright}
  \centering
   \includegraphics[width=\textwidth]{figs/detection_threshold_vs_prctile/censoring_0.3/combined.pdf}\par
   \subcaption{{30\% censoring threshold}}
   %\caption*{{Angry Birds game + click fraud}} 
   \label{fig:detect_vs_prctile_0.3_censoring}
%   \end{flushright}
\end{minipage}
\begin{minipage}[tbp]{0.3\linewidth}
  \centering
%   \begin{flushright}
   \includegraphics[width=\textwidth]{figs/detection_threshold_vs_prctile/censoring_0.5/combined.pdf}\par
   \subcaption{{50\% censoring threshold}}
   \label{fig:detect_vs_prctile_0.5_censoring}
%   \end{flushright}
\end{minipage}
\caption{(Wikipedia) Detection threshold vs robustness threshold $\gamma$. In this experiment we lower detection rate by decreasing confidence of GD's results. We consider three types of censoring thresholds: 0\%, 30\%, 50\%.}
\label{fig:detect_vs_prctile}
\end{figure*}


Standard hypothesis testing theory implies that under appropriate independence
assumptions, the probability of error decays exponentially in sample
size. To ensure that the probabilities of error goes to zero, it follows that
the sample size needs to scale logarithmically in network size ($e^{-\alpha
\log(n)} \to 0$ as $n \to \infty$). In a network of mobile applications,
{\it a priori}, it is not clear if independence across samples holds, or even a
weaker condition such correlation decay across samples holds (which also can
lead to exponentially decaying bounds).


%\sanjay{please, rewrite the text in this section}
% It can be proven that Shape GD's detection threshold scales as a logarithmic function of the number of nodes in a network while Count GD's detection threshold is proportional to the square root of the network size. Given a very large network, Shape GD can identify infected communities much faster than Count GD. Considering exponential nature of malware propagation process, even a small reduction in detection threshold can significantly reduce time to detection.

To study this, we conduct the following experiment (repeated 300 times):
we abstract away from a particular network topology because this result
should hold in a network with any internal structure. As we have described in
Section~\ref{sec:shape_vs_count}, we train Shape GD on 11,000 benign FVs.
We then run Shape GD on data sets that contain various portions of malicious
FVs (from 0\% up to 100\%) and have different sizes (from 1,000 up to 32,000).
%By varying portion of malicious FVs in a data set, we can 
We then determine detection threshold for a false positive rate of 10\%. 

%To gain statistical significance we repeat the experiment 300 times.

%When plotting the 
Figure~\ref{fig:wiki_vs_censoring_threshold} shows  detection threshold vs network size (logarithmic
scale) -- detection threshold scales down as a logarithmic function of network
size.  Specifially as we increase network size from 1,000 to 32,000, the
detection threshold drops from 19\% to 10\%. This, in turn, implies that we can
detect malware spreads at the very early stages.


% Thus, in the large communities \sysname can spot
% infection at the very early stages. Deviation from logarithmic
% dependency may have been caused by limited number of samples in our
% experiment.



==> results/pure_shape.tex <==

%\begin{figure}[tbp]
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/histogram.pdf}\par
%\caption{\textit{(Wikipedia app) Distribution of Wasserstein distances between FPs/TPs and a reference histogram. Shape-based GD can reliably separate FPs and TPs through extracting information from the data that has been unutilized by an LD.
%*The constant offset -- 8,948,200 -- has been subtracted from the Wasserstein distances.}}
%\label{fig:histogram}
%\end{figure}
%

\begin{figure*}[t]
\begin{minipage}[tbp]{0.24\linewidth}
  \centering
   \includegraphics[width=\textwidth]{figs/histogram/histogram_walmart.pdf}\par
	\subcaption{Walmart app}  
%%   \label{fig:histogram_walmart}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
  \centering
   \includegraphics[width=\textwidth]{figs/histogram/histogram_avg.pdf}\par
	\subcaption{AVG app}  
%%   \label{fig:histogram_avg}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
  \centering
   \includegraphics[width=\textwidth]{figs/histogram/histogram_buzzfeed.pdf}\par
	\subcaption{Buzzfeed app}  
%%   \label{fig:histogram_buzzfeed}
\end{minipage}
\begin{minipage}[tbp]{0.24\linewidth}
  \centering
   \includegraphics[width=\textwidth]{figs/histogram/histogram_yelp.pdf}\par
	\subcaption{Yelp app}  
%%   \label{fig:histogram_wiki}
\end{minipage}
\caption{(Wikipedia app) Distribution of Wasserstein distances between FPs/TPs and a reference histogram. Shape-based GD can reliably separate FPs and TPs through extracting information from the data that has been unutilized by an LD.
}
\label{fig:histogram}
\end{figure*}


A key property our framework builds on, is the fact that \textit{the distributional shape of true positive feature vectors differs from that of false positives}. We build here on the discussion initiated in Section \ref{sec:intro} and the results displayed in Figure \ref{fig:intro-histogram}. 

%Recall our discussion in Section~\ref{sec:ideas}: the discriminating
%power of the feature vectors is more than that of alerts. We now
%quantify if this observation can be used by a Global Detector.


% Thus,
% they leave behind a lot of unutilized information.  \todo{cut
%   candidate. Or, fold content into algo section.}

%To quantify the separation between FPs and TPs that Shape GD is able to
%achieve
In our experiments, we sample uniformly from random two subsets of feature
vectors -- one subset from a benign data set and the other one from a malicious
data set.  Each subset contains 3,000 unique feature vectors.
% i.e.  they are sampled without replacement. 
After passing these two subsets through an LD -- the Random Forest trained on both benign and malicious system call histograms -- we obtain a collection of false positives (FPs) and true positives (TPs) for the chosen subsets. We then compute the community score described in Section \ref{sec:model}. Recall that this is the Wasserstein distance between the FPs obtained in the previous step, and a uniform reference vector-histogram; and then the same thing for the TPs. To insure statistical significance of our results, we repeat this exact experiment 500 times, and then represent the histogram of Wasserstein distances as two normalized histograms in Figure~\ref{fig:histogram}.  We note that for convenience of the display, we have subtracted a large constant ($10^5$) from both FP and TP Wasserstein distance histograms -- our tests are translation invariant, so clearly this has no effect on their performance or significance.

The non-overlapping distributions (Figure~\ref{fig:histogram}) indicate that our shape-based GD (we call this Shape GD for short) can indeed separate FPs from TPs. We only show the results for four apps, but Shape GD achieves similar completely separable distributions for 8 of 10 apps in our test -- Yelp and eBay yield partially overlapping distributions which lead to some false positives and negatives in the Shape GD's output. 

The distance between the distributions varies across the apps -- Wikipedia has
the largest separation (Figure~\ref{fig:intro-histogram}) while Walmart's distributions have smaller separation -- however, as long as they can be separated, the performance of Shape GD is unchanged.

As an interesting side note, we observe that the relative distance of the FP and TP distributions from the uniform distribution is not fixed -- the only key is that these distances are different. Indeed, the order depends on an underlying app and LD's properties -- for example, Wikipedia's false positive distribution is closer to the reference vector-histogram, whereas for AVG, Walmart, Buzzfeed and other apps TPs are closer to the reference histogram.

%However, the order of distributions is irrelevant to the GD's detection results
%-- GD only needs to separate TPs and FPs from each other.
%this property of our algorithm does not interfere with its detection results.

To summarize, our experiments with multiple real-world mobile apps  
%we have empirically
confirm that the Shape GD is an accurate and robust method for
distinguishing LD's outputs into true and false positives.

%The large gap between two distributions on the Figure~\ref{fig:histogram} witnesses Shape GD's ability to separate FPs and TPs. Shape GD achieves similar results for all the apps in our corpus, i.e. it can reliably separate LD's TPs and FPs. The only difference across all the experiments resides in the relative order of two distributions. For example, Wikipedia's false positive distribution is closer to the reference vector-histogram. Nevertheless, AVG, Walmart, Buzzfeed and other apps have reverse order of the distributions.

%After choosing an appropriate LD, we proceed to the next logical step -- designing a global detector (GD) for aggregate analysis of alerts raised by LDs.
%
%As we mentioned before, the key difference with the other previous work on CIDS~\cite{seurap, survey ...} resides in the type of information being processed by GD. In comparison to the state-of-the-art CIDS, Shape GD does not aggregate LDs alerts (binary LDs' outputs) -- it reanalyzes feature vectors causing alerts. Also, Shape GD does not need to know the global network topology (e.g. size of a network at every moment of time, possible connections between all nodes and etc) -- local network topology (1-hop neighborhoods) is enough to efficiently detect malware in a community.
%
%When analyzing Shape GD, the first question we want to address is how well Shape GD separates LD's false positives and true positives. 

%To analyze Shape GD's ability to distinguish between FPs and TPs, we do the following experiment: we sample two groups of feature vectors 500 times -- one group from a benign data set and the other one from a malicious data set. Each group contains 5,000 unique feature vectors, i.e. they are sampled without replacement. However, individual benign/malicious groups may overlap. After passing these two groups through an LD, we obtain its FPs and TPs. Then for each FP/TP set we compute Wasserstein distance between the set and the uniform reference vector-histogram. As a result of this experiment, we collect 500 distances between FP/TP sets and the reference histogram, which we represent as a normalized histogram to obtain an empirical estimation of FP/TP distributions (Figure~\ref{fig:histogram}). 
%
%The large gap between two distributions on the figure~\ref{fig:histogram} witnesses Shape GD's ability to separate FPs and TPS. From information-theoretic point of view, we can say that Shape GD is able to extract the information from the underlying data that has been missed by an LD. In the experiments with all the apps in our corpus, we have observed similar results, i.e. Shape GD can reliably separate LD's TPs and FPs. The only difference is which of the two distributions is closer to the reference vector-histogram. For example, for Wikipedia's distribution of FPs is closer to the reference vector-histogram. Nevertheless, AVG, Walmart, Buzzfeed and other apps lead to the reverse arrangement of the distributions.


%Such an approach does not work in the setting where the exact number of nodes in a network fluctuates over time. In many cases, we cannot model such fluctuation, thus we have no estimate of the expected number of nodes in a network. Consequently, classic GD is not able to distinguish between malware spread and fluctuations of the number of false positives due to constantly changing size of a network.

%To overcome such a shortcoming, we have designed a network-oblivious GD. It does not need to know the global topology (e.g. size of a network at every moment of time, possible connections between all nodes and etc). As has been mentioned in the~\ref{algo sec}, our GD needs to have access to the original feature vectors that resulted in alert and local network topology -- 1-hop neighborhood. In this section we compare performance of our GD with classical approach -- count-based GD.

%In this section we compare performance of Shape GD with classical approach -- count-based GD.

%Another, and perhaps more insightful, way of looking at this is to consider the (empirical) probability mass function the feature vectors filtered in two different ways (i) the pmf of feature vectors that correspond to the true positives (real malware activity) of the local detector, and (ii) the pmf of feature vectors that correspond to the false positives of the local detector (misclassifications by the
%local detector). Information theoretic arguments in the higher dimensional feature space – effectively they have different shapes. However, their binary projections in the local detector output space is the same, thus the local detector does not (statistically) distinguish between these two collections. This points toward 
%eigen-filtering -- hypothesis testing in the feature vector space -- instead of simply aggregating outputs of the LDs.

%It is not surprisingly that the distribution of distances between FPs and the reference histogram is shifted to the left because we build a reference histogram to roughly approximate this distribution. In this setting the distances between TPs and the uniform histogram are no less than the distances between FPs and the reference histogram. 



%\begin{figure}[tbp]
%   \centering
%   \includegraphics[width=0.45\textwidth]{figs/pure_shape/NO_censorship_w_10_prctile_10.pdf}\par
%%\caption{\textit{(Wikipedia) Detection rate scales as log of the number of nodes in %the network.}}
%\label{fig:shape_vs_count}
%\end{figure}
%
%\begin{figure*}[t]
%\begin{minipage}[tbp]{0.3\linewidth}
%%   \begin{flushleft}
%   \includegraphics[width=\textwidth]{figs/pure_shape/censorship_0_3_w_10_prctile_1.pdf}\par
%   %\caption*{{} }
%   \label{fig:count}
%%   \end{flushleft}
%\end{minipage}
%%\hfill
%\begin{minipage}[tbp]{0.3\linewidth}
%%   \begin{flushright}
%   \includegraphics[width=\textwidth]{figs/pure_shape/censorship_0_3_w_10_prctile_10.pdf}\par
%   %\caption*{{Angry Birds game + click fraud}} 
%   \label{fig:ab-2}
%%   \end{flushright}
%\end{minipage}
%\begin{minipage}[tbp]{0.3\linewidth}
%%   \begin{flushright}
%   \includegraphics[width=\textwidth]{figs/pure_shape/censorship_0_3_w_10_prctile_30.pdf}\par
%   %\caption*{{Angry Birds game + click fraud}} 
%   \label{fig:ab-2}
%%   \end{flushright}
%\end{minipage}
%\caption{(Wikipedia) Effect of percentile threshold}
%\label{fig:pure_shape}
%\end{figure*}
%
%
%First, we compare detection rate of Shape and Count~\ref{fig:shape_vs_count}. In this experiment, we use normalized histograms for the Shape detector. Shape starts working at 14.4\% level, while Count starts working at 3.8\%. The error bars correspond to 10 and 90 percentile respectively.
%
%Second, we compare the effect of threshold (aka percentile parameter) on detection rate. When varying the detection confidence (consequently, FP rate) from 1\% to 30\%, detection changes from 27\% to 3.7\%~\ref{fig:pure_shape}


==> results/shape_vs_count.tex <==
\begin{figure*}[t]
\begin{minipage}[tbp]{0.33\linewidth}
  \centering
%   \begin{flushleft}
   \includegraphics[width=\textwidth]{figs/count_vs_pure_shape/no_censoring/random.pdf}\par
   %\caption*{{} }
   \subcaption{Random graph}
   \label{fig:shape_vs_count_random}
%   \end{flushleft}
\end{minipage}
%\hfill
\begin{minipage}[tbp]{0.33\linewidth}
  \centering
%   \begin{flushright}
   \includegraphics[width=\textwidth]{figs/count_vs_pure_shape/no_censoring/grid.pdf}\par
   %\caption*{{Angry Birds game + click fraud}} 
  \subcaption{Grid graph}
   \label{fig:shape_vs_count_grid}
%   \end{flushright}
\end{minipage}
\begin{minipage}[tbp]{0.33\linewidth}
  \centering
%   \begin{flushright}
   \includegraphics[width=\textwidth]{figs/count_vs_pure_shape/no_censoring/social.pdf}\par
   %\caption*{{Angry Birds game + click fraud}} 
   \subcaption{Real network}   
   \label{fig:shape_vs_count_social}
%   \end{flushright}
\end{minipage}
\caption{(Wikipedia) Shape GD vs Count GD. 
%(Count vs Shape -- no Censoring) Random -- Grid -- Social graphs (10\% percentile)
}
\label{fig:shape_vs_count}
\end{figure*}

We refer to Count GD as the algorithm that relies on increased
alert-count inside specific communities, in order to declare a global
infection (see also \cite{Dash2006,Seurat2004} for related approaches). In contrast to Count GD, our approach, Shape GD, does not critically need the number of nodes in the network. Indeed, when this information is not available, {\em Count GD cannot work}. But if we do have this information, the idea of Count GD can be useful. In this section, we compare Shape GD and Count GD in the setting most favorable to Count GD -- fixed and known graph topology. Our results show that even here, Shape GD does almost as well as Count GD. This suggests that in cases where we can reasonably expect to know the graph (and hence the total number of nodes), combining Count GD and Shape GD would give the best results. On the other hand, if the total number of nodes is not known, Shape GD is our only recourse.

We now describe in detail our experiments that lead to the results summarized in the previous paragraph. We quantify the ``price'' of such flexibility by comparing Shape and Count GDs' detection accuracy by running them on a random network, a grid, and a social network.

\ignore{
The training procedure for Shape GD and Count GD is identical: 1) choose a
low-dimensional basis; 2) project benign training data set onto the chosen
basis and compute LD's false positives; 3) appropriately discretize the data
and convert it into vector-histogram representation; 4) compute community
score; and 5) define a {\em detection threshold} for the GDs by fixing a 
false positive rate. }
%error
%bound.\todo{check for consistency: error bound -- false positive}


We allocate a training data set of 11,000 benign feature vectors (FVs) for each
app (i.e., over 3 hours of real usage per app).  To represent data in the form
of vector-histograms we need to determine optimal disretization, i.e., the
number of bins and their edges.
%These parameters are associated with a GD and once being set, they never get
%updated. 
We choose these parameters by passing the benign training set FVs through LDs
on each node to obtain false positive FVs, remove points below and above
1\%/99\% percentile respectively, and choose the number of bins proportional to
the square root of the number of suspicious samples.  Experiments show that 50
bins is an adequate number since the number of suspicious feature vectors is
around 2500 (out of 11000 samples, based on the LD's false positive rate).  We
then add two extra bins to represent data points below the lower bound and
above the upper bound.

Note that a GD is not constrained to use the same basis as LD. 
In our experiments, 
%we use different bases for both. 
although both GDs and LDs use the same FE
algorithm -- histogram of system calls -- and apply PCA to reduce
data to 10 dimensions,  GDs receive only the feature vectors that
lead to alerts by LDs. 
%and projects all suspicious feature vectors on top 10
%principal components.

The actual training procedure consists of 300 iterations. On each iteration we
sample without replacement a subset of 5,500 feature vectors from the
previously allocated set, pass it through an LD, obtain false positive FVs,
project them on the basis chosen above, discretize using the corresponding
bin edges, and compute a community score for the chosen FV-subset. We
repeat this iteration 300 times to determine the range of
community scores (based on the parameter $\gamma$ in Section~\ref{sec:model})
outside of which the GD declares a community as infected.
GDs thus act like anomaly detectors, and the key difference between Count and Shape 
GDs is that Count relies on the number of alerts, where as Shape GD goes back to the feature vectors and then uses the Wasserstein distance community score.

\ignore{
if its
score is outside the range. The range depends on the confidence parameter
$\gamma$ (sec.~\ref{algo_description}). In our case the upper bound of the
range is defined as $\gamma/medium FP-Score$ percentile, by analogy the lower
bound is $(100-\gamma)/medium\ FP-Score$ percentile. Thus, if in the deployment
mode GD finds a community score to be outside the range and labels a community
as infected, then the expected probability of error is $100-\gamma/medium\
FP-Score$. Count GD's training procedure is almost identical -- instead of
capturing the shape of false positive distribution, it captures the number of
alerts.  \mikhail{i could formally describe this if we need}
}

After training Shape and Count GD, we run both detectors on the three networks
and show the results for Wikipedia in 
%networks with different topologies:  random graph, a grid graph, and a social
%network 
Figure~\ref{fig:shape_vs_count}. The plots in the top row characterize
performance of Shape GD, while the ones at the bottom show behavior of Count
GD. The horizontal axis depicts infection rate (ground truth), i.e., the number
of infected nodes in a network, the vertical axis plots community scores. The
blue line shows the average community score for benign FV-sets obtained during
the training procedure. The red line corresponds to the community score
assigned to the groups of suspicious FVs. We set false positive rate $\gamma$
to be 10\% of  for each experiment. To show this
(Figure~\ref{fig:shape_vs_count}), we draw error bars that correspond to 10\%
and 90\% percentile community score values. For each discrete step in the
malware propagation process, we compute the community score of suspicious FVs
sent by LDs to GD for classification. Thus the earliest time step at which the
red curves 
achieve complete separation from the blue curves 
determines the GD's {\em detection threshold} (in terms of number of compromised nodes).

When comparing GDs' performance on random and grid networks, we see that grid
structure results in earlier detection (Shape GD: 8.8\% and 4.6\%; Count GD:
8.8\% and 3\% respectively) due to high and regular local connectivity.  In the
social network graph, Shape GD achieves the worst performance -- 14.4\% across
all network topologies, while the Count GD starts detecting malware at 2.4\%
level (the best result for Count GD). %This difference may be caused by \todo{Why?}.

In summary, the robustness of Shape GD leads to a higher detection threshold in
comparison to Count GD. Hence, it is possible to develop a hybrid GD that
incorporates both Shape and Count detectors to achieve the earliest detection
in a network with fixed topology and also cover cases when network nodes may
randomly switch on/off.

%To compare Shape GD with Count GD, %%we use both of them to detect malware spread over the network~\ref{fig:counts_vs_shape}. Even if we designed our system to be network-oblivious -- size of the network is unknown -- in this experiment we assume that network has a constant size, otherwise we would be unable to use Count-based GD.

%In this experiment, $\alpha=10%$, i.e., error bars correspond to 10- and 90- percentiles. The horizontal axis depicts infection rate, i.e., the number of infected nodes in the network. And for each discrete step in the malware propagation process we compute the community score of suspicious data transmitted by LDs to GD for classification.

%The blue line shows median distance between a group of false positives and a uniform reference histogram. The red line correspond to the community score assigned to the groups of suspicious data. Its error bars are 10- and 90- percentiles. We say that GD is able to detect malware if red and blue error bars do not overlap.

%Each subplot corresponds to one of the underlying network topologies that we consider in our experiemnts: random graph, grid graph and real social network. The subplots in the top row shows how Shape GD reacts to malware propagation, while the subplots at the bottom show the same for Count-based GD. 

%When we compare GDs' performance on random and grid networks, we see that grid structure results in earlier detection (Shape GD: 8.8\% and 4.6\%; Count GD: 8.8\% and 3\% respectively) due to high local connectivity. If compare random and grid graphs with a social network graph, we can notice that Shape GD achieves the worst performance -- 14.4\%, while the Count GD starts detecting malware at 2.4\% level. This difference may be caused by ???. 

%As malware gets propagated over the network, Count GD's malicious score grows as a linear function as one may expect. At the same time, Shape GD's malicious score resembles a logarithmic function that slowly stabilizes.



==> theory.tex <==
% Sanjay's text goes here
%\section{Formal model}
\input{theory/model}



==> todo-imp.tex <==
* fig 1 needs 'alert FVs'
* cites in first para: permissions demystified, rowhammer, stanford-accel, master-key
* constantine text citations
* consistent time to detection across all sections.








By re-analyzing alert-FVs instead of the LDs' alerts,
and specifically by grouping the alert-FVs into neighborhoods,
Shape GD is able to squeeze more information out of the alert-FVs 
than the neighborhood of LDs working separately. 
At the same time, analyzing the aggregate shape of 
neighborhoods' alert-FVs' makes Shape GD robust to
noise in estimating neighborhoods' sizes compared to prior Count GDs. 
Shape GDs' benefits thus generalize to any scenario where the LDs
are weak and the neighborhoods noisy.

This is the fundamental reason why
its FPs






* address reviews from proposal and oakland

* read paxson, kruegel, mihai, etc to match experimental setup 

* paper-ss.pdf comments on results_v3

* 100\% TP or 99\% TP: why?

* discussion: DNNs.

* discussion: other applications of nbd + shape.

* discussion: global FP. 
1\% global FP. 5\% LD FP rate, 15,000 alert-FVs ndb size,
1FV/node/sec. 1000 nodes. 1000FVs/sec. 
5\% local FP --> 50 alert-FVs/sec. 
300 seconds (5 minutes). 
1\% FP means every 500 minutes, there is 1 global-FP that needs a closer
look at the 1000 node nbd. In Count GD, all LD calc same, so 5 minutes to
produce 15k alert-FVs 


* make sure FP is 6\% NOT 5\% throughput

